EMMA: A New Platform to Evaluate Hardware-based Mobile Malware Analyses

Hardware-based malware detectors (HMDs) are a key emerging technology to build trustworthy computing platforms, especially mobile platforms. Quantifying the efficacy of HMDs against malicious adversaries is thus an important problem. The challenge lies in that real-world malware typically adapts to defenses, evades being run in experimental settings, and hides behind benign applications. Thus, realizing the potential of HMDs as a line of defense - that has a small and battery-efficient code base - requires a rigorous foundation for evaluating HMDs. To this end, we introduce EMMA - a platform to evaluate the efficacy of HMDs for mobile platforms. EMMA deconstructs malware into atomic, orthogonal actions and introduces a systematic way of pitting different HMDs against a diverse subset of malware hidden inside benign applications. EMMA drives both malware and benign programs with real user-inputs to yield an HMD's effective operating range - i.e., the malware actions a particular HMD is capable of detecting. We show that small atomic actions, such as stealing a Contact or SMS, have surprisingly large hardware footprints, and use this insight to design HMD algorithms that are less intrusive than prior work and yet perform 24.7% better. Finally, EMMA brings up a surprising new result - obfuscation techniques used by malware to evade static analyses makes them more detectable using HMDs.

==> CONFLICTS.tex <==
paper.tex:  

abstract.tex:

intro.tex:

motivation.tex:  Mohit

malware-gen.tex:Jimmy


impl.tex:       

arch.tex:

results2.tex:  

related.tex:  Mohit  

conclusion.tex:     

threat-deploy.tex: Mohit


==> arch.tex <==
We now present two types of anomaly detection algorithms -- a probabilistic
Markov model that models time explicitly, and a bag-of-words model that doesn't
and uses statistical distance instead.
%to a) ensure that our results are not a fluke of machine learning heuristics
%and b) to evaluate whether app:algorithm pairs have an effect on detection
%rate. 
Interestingly, our results show that training on real malware payloads and
benignware executions enables both of our HMDs to be simpler than prior work
(sampling counters at 80ms instead of 10k or 25k cycles).
Further, we find that for some complex apps, the simpler bag-of-words model
outperforms the Markov model with equivalent training effort.

%Markov model having two
%models 

%algorithms 
%that turn a set of time-series
%(performance counter) data into


%It is essential to extract meaningful features to represent the time series
%traces and choose appropriate models to capture the patterns in the data.
%Most of the previous representations extract local temporal or frequency
%information to characterize time series, which are very effective for short
%time series or time series with periodic waveforms. 

%\mikhail{To capture high-level structural information of long time series which have
%repetitive but non-periodic patterns, we perform time-frequency analysis on the
%data to extract program phases introduced in. And we 
%represent the temporal relations between the program phases using a state-based 
%Markov model~\cite{Phase}. We also experiment with a bag-of-word based method 
%similar to~\cite{BOW}. These two models capture apps' behavior from different 
%aspects: temporal pattern (Markov model) and statistical profile (BoW).  For 
%each model, we determine values for all numeric parameters based on an extensive 
%search of the parameter space and optimizing for the best detection results.}
%
%\ignore{
%\begin{comment}  MICRO
%To capture high-level structural information of long time series which have
%repetitive but non-periodic patterns, we perform time-frequency analysis on the
%data and use a state-based Markov model~\cite{Phase} to capture the patterns in
%the execution traces and construct computational signatures for applications.
%We also experiment with a bag-of-word based method similar to~\cite{BOW}.
%These two models capture apps' behavior from different aspects: temporal
%pattern (Markov model) and statistical profile (BoW).  For each model, we
%determine values for all numeric parameters based on an extensive search of the
%parameter space and optimizing for best detection results.
%%and describe the method and its experimental results in
%%Section~\ref{subsub:BoW}.
%\end{comment}
%}

Our anomaly detection approach 
%for detecting novel malware 
consists of three steps --  
preprocessing data, representing data using states, and building
a model for the data that is then used to label anomalous data. 
%
The performance counter traces we collected are multi-dimensional (one for
each performance counter), high frequency, and bursty time series.
%
Hence, applying these three generic steps to performance counter time-series
to yield an efficient anomaly detector is a hard problem.
%It is a challenging task to 
%efficiently and effectively analyze these data, model the
%normal behavior of the apps, and detect novel patterns resulted from unknown
%malware.  


%We discuss how we tune these steps to our 
%problem of modeling performance counter time-series and detect anomalies.

%\mikhail{We are 
%not the first to propose this combination for modeling time series data,
%but we are the first to apply such approach to modeling the execution of
%mobile apps and detecting anomalous/malicious activity.}
%
\subsection{Data Preprocessing}
We observe that the performance counter traces are usually very noisy and often 
contain large outliers that are orthogonal to our problem. Thus, before  
constructing the computational model for an application, we
remove large outliers from its performance counter traces.
%
%To remove outliers, we independently process each time
%series data from a performance counter in an application.  
%For each time series that is available for constructing the model, we
We use the 99.99 percentile of all values in the trace as the
cut-off value, and replace all the values in the trace that exceed the cut-off
value with the cut-off value.
%
After removing large outliers, we smooth the data using a moving average 
with a tunable window size {\em smooth\_window}. Our experiments show that 
{\em smooth\_window} =100 ms provides a good trade-off between removing useless 
noise from and keeping useful details in the data. After data smoothing, 
we normalize all data to the range [0,1]. 

%All parameters used in data preprocessing are saved, so that incoming new 
%data can go through exactly the same transformation.

%When we collect measurements from
%multiple performance counters, we get a multi-dimensional data matrix for the
%application, with each column (dimension) of the matrix being the time-series
%trace from a performance counter, and each row of the matrix being an observation
%from all performace counters at a specific time.
%The absolute value of the threshold i.e. the actual threshold * the mean of the dataset  and the maximum magnitude of each time-series are stored in memory, and these values are applied to the testing dataset. Mean, mad are only estimated for training dataset, for testing dataset the constant values are used. This is done to achieve invariance: if the same trace is used for training and testing, the results of its smoothing and normalization when it is included into a large training 7D time-series and when it is processed individually during testing should be roughly the same.

%There is a parameter called shift\_step that allows to artificially produce benign data by shifting benign time series by shift\_step and appending to the original data. Usually, this parameter is set to be equal to some fraction  of a phase\_window

%\mohit{we need a figure to show the data matrix with time dimension and
%signal dimension, and also show how we transform the data matrix into
%the wavelet based feature representation.}

\subsection{State Representation of the Data}
\label{sub:representation}

Due to the noise and transient variations in the time series, we do not
construct our models directly from individual raw values of the traces.
Instead, we use program phase analysis techniques~\cite{Phase,BOW},
specifically
%use an approach similar to~\cite{Phase, BOW} to
Discrete Wavelet Transform (DWT) and $k$-means clustering, to derive states 
for the Markov model and the codebook for the bag-of-words model.

%We then uses these states (i.e. phases) to build a Markov model or 
%The state representation of the traces forms the basis for the states used in
%our Markov model and for the codebook used in our bag-of-word model.

\noindent{\bf Feature extraction.} We divide the long time series traces into
short segments and extract a feature vector from each local segment using the
DWT.  Specifically, we organize a multidimensional trace into a matrix, with
rows denoting measurements over time and columns denoting measurements from
different performance counters.
%
We then continuously slide a time window with a predefined length specified by
the parameter {\em state\_window}, which is typically in the range of 50ms to
150ms, along the rows of the matrix to extract a set of local segments (i.e.,
submatrices) and order them by the starting time of the window. We then perform
a 2D DWT on the local segments, and use the approximation wavelet coefficients
of the DWT to form a feature vector to represent each local segment.

%The key parameters of in the transformation include wavelet approximation level 
%{\em wavelet\_level} (typically from 2 to 5) and wavelet type {\em wavelet\_type} 
%(typicall Haar or Daubechies).
%
%For each one-dimensional time series in a
%multidimensional trace, we use a sliding window with pre-defined
%length to extract a set of local segments and order them by the
%starting time of the window. We then transform each local segment into 
%wavelet domain and use the approximation wavelet coefficients of
%Discrete Wavelet Transform (DWT) as a feature vector to represent the local segment. 
% 
%Then, after we get all the feature vectors from local segments from the same
%sliding window but across different dimensions, we concatenate their
%feature vectors together into single one to represent the 
%multidimensional trace from this sliding window.

The wavelet transform can provide both accurate frequency information 
at low frequencies and time information at high frequencies, which are 
important for modeling the execution behavior of the applications.
%The choice of wavelet function and the number of decomposition levels is of importance for the
%multiresolution decomposition. 
We use a three-level DWT with
an order 3 Daubechies wavelet function (db3) to decompose a
local segment. We also used the Haar wavelet function, but did not observe
much difference in the detection results.
A similar approach has been shown to be 
effective in modeling a variety of time series data~\cite{ECG, BOW}.

\mikhail{In comparison to ~\cite{anomaly-detector-columbia-raid} and ~\cite{perf_counters_2013}, we use 
a principally different feature extraction schema. First, each feature 
vector in our case is 10-150 times longer than in~\cite{anomaly-detector-columbia-raid}. 
Second, the sampling frequency is approximately 3-4 orders of magnitude 
lower in our experiments. 
Due to the large number of samples aggregated within 
individual feature vectors, we believe that DWT is more adequate for 
filtering out the noise than statistical methods such as power transform~\cite{anomaly-detector-columbia-raid}.
}

\noindent{\bf State formation.}
With the feature vector representation of traces, we use the $k$-means method
to compute $m$ representative states for the traces. 
%and only the number of states through experiments.
% 
Specifically,
we perform $k$-means clustering with $m$ clusters on feature vectors derived 
from all benign traces in the training set, and use 
the centroids computed by $k$-means as the state codebook for the traces. 
%Suppose a group of local segments $X = [x_1, ~ x_2, \ldots, x_n]$,
%where $x_i \in R^d$ , are feature vectors of local segments 
%extracted from the time series traces. Then we learn from feature vectors 
%a state codebook $S \in R^{d \times m}$ with $m$ states, each of which is 
%a $d$-length vector, the same length as the local segments. 
Note that we do not define the states apriori. Instead, we derive the states from 
the benign apps' traces. Also,
we only need to learn these states once from training data
because they are universal for both training and test data.

Note that the current algorithm used for state formation does not guarantee a
direct mapping between human-level states (e.g.  staying on the same webpage
and reading news) and the states in the Markov model. This is because one high-level
state may correspond to a chain of low-level states derived from the app's code
and microarchitectural data. 

\ignore{
The codebook size K is of importance to the bag-of-words
representation. A compact codebook with too few entries has
a limited discriminative ability, while a large codebook is
likely to introduce noise due to the sparsity of the codewords
histogram. Therefore, the size of the codebook should well
balance the trade-off between discrimination and noise.

We next perform $k$-means clustering on feature vectors derived from all traces
of an application that are available for training. We experiment with a variety
numbers of clusters, and find using $k=1000$ clusters giving a nice trade-off
between the representation quality the wavelet coefficients. 
Since the size
of the transform is 16×16, our data have 256 dimensions.
The number of points to be clustered is the number of in-
tervals in the program. The distance between two points
is the Euclidean distance between their wavelet coefficients,
but we first apply tuning weights to the coefficients using
a scheme similar to [13] because the importance of a coeffi-
cient is affected by its 2D position. The result of k-means is
that every interval in the program has been assigned to one
of ten clusters.


Each state $c_i$ is a multidimensional vector, and 
is indexed by a number $i$. Then the chunk of the 
original multidimensional trace can be indexed by a state, which is the 
centroid/state number closest to vector of it wavelet coefficients. 
%with a set of clusters i.e. with the set of centers of the obtained clusters. 
Then, the whole muti-dimensional time-series trace is encoded as a sequence of 
state numbers, each of them is a number of a centroid that best approximates 
the data.
}
%We do kmeans clustering 6 times starting from a set of random initial clusters. We choose the replicate parameter to be equal to half the size of matlab thread pool (i.e. 6 because matlab thread pool = 12). Ling, I use the C-code for kmeans; the one you sent to me. And I use default parameters; if you are going to mention anything about that code, you can refer to the default parameters.

\noindent{\bf State assignment.} Once the state codebook is constructed,
the local segments within a trace are assigned to the state whose
feature vector has minimum Euclidean distance from the segment.
Specifically, suppose that a codebook with $m$ entries, $S = \{s_1 , s_2 , ..., s_m \}$, 
is learned from the training data. A local segment $x_i$ is assigned
the $c^{th}$ codeword that: $c^{\ast} = argmin_j d(s_j , x_i)$, where $d(\cdot, \cdot)$
is the Euclidean distance function.

In addition to the state codebook for all the observed states, 
we also have an alphabet for the unobserved states. When a malware 
execution introduces a new state that is not well represented 
by the observed states, we will assign it the alphabet for the 
unobserved states.

\ignore{
For a chunk of multidimensional time-series, which is a sub-matrix of
size $t \times d$, where a row contains measurements from all
performance counters at a given time, and a column contains all
measurements from a performance counters over time, we convert it into
a single vector of size $p$, which is determined by $t, d$ and the
wavelet approximation level $l$ (typically from 2 to 5). 

For each column of data, we do the one-dimensional wavelet 
transformation at an approximation level $l$, using either Haar or
Daubechies wavelet, to compute its wavelet coefficients. We then
concatenate the ???? coefficients across different columns into a single vector.
In this way, we transform a sub-matrix of multidimensional data from a time 
window into a single vector (of wavelet coefficients).
}

%-------------------
\begin{figure*}[t] 
   \begin{minipage}[tbp]{0.24\linewidth}   
	   \includegraphics[width=\textwidth]{figs/pca-benign.pdf}\par
	   \label{fig:pca-ut-benign}
   \end{minipage}
   \begin{minipage}[tbp]{0.24\linewidth}
      \includegraphics[width=\textwidth]{figs/AngryBirds_phase_tp_vs_phase_fp.pdf}\par
      \label{fig:ab-v-rest}
   \end{minipage}
%\hfill
   \begin{minipage}[tbp]{0.24\linewidth}
      \includegraphics[width=\textwidth]{figs/Sana_phase_tp_vs_phase_fp.pdf}\par
      \label{fig:sana-v-rest}
   \end{minipage} 
   \begin{minipage}[tbp]{0.24\linewidth}
      \includegraphics[width=\textwidth]{figs/Radio_phase_tp_vs_phase_fp.pdf}\par
      \label{fig:radio-v-rest}
   \end{minipage}    
  
%   \caption{Benign apps plotted in the PC space.}
   \caption{(Left plot) PCA analysis of baseline apps' instruction mix. (3 right plots) Difference among 3 representative 
	baseline applications obtained with the Markov model by training on one app and testing on the rest two apps. 
	Based on PCA analysis, we can conclude that the baseline apps form a diverse set. The Markov model justifies 
	the behavioral difference observed on the microarchitectural level.} 
   \label{fig:baseline-diff}
\end{figure*}
%-------------------


\subsection{Markov Model HMD}

Our first approach to constructing models for benign apps is based 
on the first-order Markov model. This assumes that the normal execution of an 
application (approximately) goes through a (limited) number of states 
(program phases), and 
the current state depends only on the previous state. The goal is to detect 
malware if its performance counter trace creates 
%if malware
%is interleaved into a benignware execution, it will exhibit a 
a sequence of rare state transitions (as shown in Figure~\ref{fig:ab}). 

\mikhail{Thus, Markov model is supposed to learn probable state sequences. 
Our assumption is that malware changes the state sequences of the underlying app, i.e. 
perturbs the states of the underlying app, giving a raise to low probable 
state sequences. If malware introduces a new state, the malware execution 
exhibits a sequence of states that largely deviates from those of benign apps. 
The more intensive malware is, the lower probability is
the sequence, and the more likely the Markov model is to raise an alarm.}
%The entire process of constructing 
%of the Markov model based signature consists of the following stages:
%1) state representation of the traces, 2) construction of Markov model on states,
%and 3) detection using Markov model.

\noindent{\bf Construction of Markov model.}
% To capture important state transitions in the application execution, we 
% train our Markov model with a small number of states using benignware traces.
%execution traces under normal conditions.
%We specify a small number of clusters to $k$-means when we 
%use it to compute states from the traces. 
The number of states is equal to the number of clusters in $k$-means algorithm (as we
describe above), 
and we used the Bayesian Information 
Criterion (BIC) score~\cite{Pelleg-xmeans} to find that 10 to 20 states
is a good number. 
%This is similar to previous work~\cite{Sherwood-large-scale-behavior} 
%on program phase detection.
% and multiple experiments with different parameter settings.}
%
We then build a first-order Markov model 
based on the states we derived. For a model with a finite $m$ number of 
states, the stationary Markov model can be defined by a $m \times m$ transition 
probability matrix $P = [p_{ij}]$ for $i,j = 1 \ldots m$, and an initial probability 
distribution $Q = [q_1 \quad q_2  \quad \ldots \quad q_m]$~\cite{Markov}.

Using a sequence of observed state transition derived from the multi-dimensional 
trace data, we can estimate the transition matrix $P$ and initial
probability distribution $Q$ empirically using training data using a
Maximum Likelihood Estimation (MLE) method~\cite{Markov}. 
The transition probability $p_{ij}$ between state $i$ and $j$ is defined as
%\begin{equation}
$p_{ij} = Pr(s_{t+1} = j|s_t = i)$.
%\end{equation}
Then the MLE estimation of $p_{ij}$ is
%\begin{equation}
$\hat{p}_{ij} = {n_{ij}}/{\sum_{j=1}^m n_{ij}}$,
%\end{equation}
where $n_{ij}$ is the number of observation pairs of state $i$ and state $j$. 
%Based on the approximation obtained on the previous step, we build a Markov chain. 
%In other words, we estimate conditional and initial probabilities empirically. 
%The size of the matrix that represents the Markov chain is equal to
%the number of clusters.

\mikhail{To robustly estimate all probabilities under limited observations, 
we use heuristics to set several transition probabilities (instead of estimating 
from data). For example, we set self-transition probabilities $p_{ii}$ to 
be a small value (e.g., 0.2). This setting intuitively captures the 
bursty usage pattern of a user on an app: the application
is either in idle mode for a while, or used by an user for a while.}
%I use a “hack” to account for the event-driven model of Android applications: the probability of self-edges in the Markov chain is initialized by fixed small values (ex. 0.2). This says that if an app stays in the state, this activity does not look suspicious. Usually, malware does not have an event-driven nature, so it needs to transition between states. While assigning fixed probabilities to self-edges also reduces the amount of input data we need to train the model. 

%For example, we may obtain two traces generated by the same user by executing the same sequence of user events, but delays between events are different. If we use fixed probabilities for self-edges, then the traces are equivalent for the training purposes; and we need only one trace, not both. Experimentally, it has been proven that such a modification of the canonical Markov model is reasonable.

%The current phase (building markov model) has the following parameters: boolean use\_initial\_probabilities, Boolean use\_fixed\_probabilities\_for\_self-edges, fixed\_probability (this parameter is assigned to a self-edfges). 

%\mikhail{we can estimate Q based on the input data (?)}

%\mohit{We estimate the initial probability distribution $Q$ from the training 
%data set. 

%When we turn off the usage of initial probabilities, we assume uniform prior distribution. The use of fixed probabilities for self-edges may be also turned off. Usually, we use initial probabilities in our model and also we assign fixed probabilities to self-edges (0.2-0.3)

\noindent{\bf Detection using markov model.}
%\label{Sec:detect-markov}
With a trained Markov model, we can perform near real-time detection using
traces in the field (or on the testing set). 
%
%When performance traces are collected continuously, we take a 
The detector pre-processes a
time-window long multidimensional trace data as we described above
to determine the current state (or phase) the app is in.
%of size {\em state\_window} in sequence. 
%For each segment, we perform the data preprocessing and compute its state representation $s$.
%With a sequence of $k$ trace segments, we obtain 
By recording 
a {\em sequence} of execution 
states $s_1, ... , s_k$ of the trace, 
%According to Markov property, 
the detector can compute the probability that 
this sequence occurs in the context of the learned Markov model as:
\begin{equation}
Pr(s_1, \ldots, s_k) = q_{s_1}\prod_{t=2}^kp_{s_{t-1}s_t}.
\end{equation}
%Intuitively, a malware usually does certain executions that a normal application
%rarely does. In such a case, malware execution may go through a 
%set of states that the application normally rarely go through. 
The detector tracks this probability value over time and 
if malware computations create anomalous hardware signals, this 
probability goes low.
%When the trace segments continuously come in over time $t$, we update the 
%probability over time and obtain a probability curve.
To further de-noise the performance counter data,
%and add certain second-order property to the Markov model, 
we smooth the probability curve using a moving average filter.
%to add kind of a “voting” rule. 
%Our intuition is that, 
Finally, since most atomic malware actions require time longer than a few 80ms to 100ms
time windows, instead of using a single value to raise an alarm,
% as an indicator 
%of suspicious activities, we use the average of neighboring probability values
%as the indicator of anomalous behavior. Using the smoothed probability, we 
we raise an alarm when more than five consecutive probability values are below a 
threshold (that we specify). Five time windows are thus the minimum time to detection
for our Markov model.

%these parameters have to be trained for each benign app.


%During the online detection, we compute joint probability per detection window, and then shift it by one {\em state\_window}. So, we get a probability value per 
%{\em state\_window} size of data using all the data in the detection window, i.e.,
%two adjacent probability values over time are computed using overlaping data. 
%In this way we obtain a probability curve. 
%We expect the execution of malware usually go through low probability states and make low-probability transitions in the context of the given Markov model, so its probability should go low.


%We estimate our confidence in the decision based on how far the current threshold is from the normal distribution that we fit to the benign traces during training phase.
%The other way to do detection is to fit a normal distribution to chunk of probability curve and estimate the distance between the just-fit normal distribution and the normal distribution fit to the benign traces during the training phase.
%Our confidence in a particular decision is based on two factors: time and magnitude. The parameter time defines how long a malware stays below a threshold (longer it stays below the threshold, more confident we are). Magnitude specifies how far a malware on a probability scale from the Normal distribution that have been fit to benign traces.

%9. Miscellaneous 
%The model may be used to measure the similarity of dynamic behavior of two different apps. For example, this is demonstrated in the case of slightly different malware samples (semantically equivalent malware, but they have differnet intensity)


\subsection{Bag-of-words HMD}
\label{subsub:BoW}

Our second approach to modeling benign applications
%constructing computational signatures is based on 
%bag-of-word model similar to ~\cite{BOW}.
%In a nutshell, this model 
%is very similar to modeling a dataset of text documents --
%the word representation of a document: 
treats a time series trace
like a document that consists of a set of representative
words (states). While simple, this bag-of-words model has been successfully
applied to a variety of tasks in text mining~\cite{BOWTEXT}, computer vision~\cite{BOWCV} 
and time series analysis~\cite{BOW}. Our results in Section~\ref{sec:results} 
show that this simple model works well, and sometimes better than even the Markov model,
in detecting malware as anomalies.

%email spam detection, information retrial,  computer vision object
%recognition. 

%Wang, Jin, Liu, Ping, She, Mary F.H., Nahavandi, Saeid and Kouzani,
%Abbas 2013, bag-of-words representation for biomedical time series
%classification, Biomedical signal processing and control, vol. 8,
%no. 6, pp. 634-644. 

%Finding Structural Similarity in Time Series Data Using Bag-of-Patterns Representation
%Jessica Lin and Yuan Li

%J. Sivic and A. Zisserman. Video Google: A text retrieval approach to
%object matching in videos. In ICCV, 2003.

%D. Nister and H. Stewenius, "Scalable recognition with a vocabulary
%tree," in CVPR '06.

The codebook size $m$ is an important parameter in the bag-of-words
model. A compact codebook with too few entries has
a limited discriminative ability, while a large codebook is
likely to introduce noise.
Unlike using 10-20 states in the Markov model, we use $m = 1000$
codewords in the bag-of-words model, which 
balances the trade-off between discrimination and noise well.

It is straightforward to construct the bag-of-words representation of
a trace. We perform the same data preprocessing and state representation
on the trace as in the Markov model, but mapping trace-segments to one of $m$ codewords.
After each local segment of a trace is assigned a codeword, we ignore
the temporal order of local segments, and represent the trace by a histogram
of size $m$. 

%The vector contains the histogram of codewords 
%in the trace, each entry of which specifies the count of a codeword occurring in the trace. 

With histograms to represent benign traces, we 
train a one-class SVM model~\cite{OCSVM} to represent the application.
One-class SVM is a widely used novelty detection algorithm. Intuitively, it aims to find
a minimum nonlinear region that can enclose most of the benign states, and classify the 
states outside the region as anomalies.
Bag-of-words differs from the Markov model since it discards
state transitions in favor of a histogram of larger number of states.

\ignore{
1. Given a {\em time to detection} window, divide the long time-series
along time dimension into multiple segments, each of size  {\em time to detection} 
2. Inside each segments, we use a moving window of
size {\em state\_window} along the time dimension to get chunks of
data. The shift of the moving window is defined by {\em shit\_step}, so
the consecutive chunks diff by a window of {\em shit\_step}, which is
usually a fraction of {\em state\_window} size.
%There is a parameter called shift\_step that allows to artificially
%produce benign data by shifting benign time series by shift\_step and
%appending to the original data. Usually, this parameter is set to be
%equal to some fraction  of a phase\_window
3. Wavelet feature extraction
4. Clustering chunks
5. Construct codebooks
6.  Fore each segment, assign codebook to each chunks in it and
compute the histogram of the codes in the segment

The main steps of a bag-of-words approach are as follows. 
0. Preprocess the data as we discussed before (with some modification)
1. Divide the long time series into short ones using either expert
knowledge (e.g., based on user action) or pre-defined
time-to-detection length TTD
(e.g., split the 10-min long traces into 5-sec long traces)

2. Each short series is a unit of detection, and will be treated as an
observation sample (akin a text document).

3. Treat all the short time series as independent documents, use an
approach similar to Fig. 1 as the following paper to build the
bag-of-words model.

Bag-of-words Representation for Biomedical Time Series Classification.
Jin Wang, Ping Liu, Mary F.H.She, Saeid Nahavandi and Abbas Kouzani.

Specifically, the main steps for bag-of-word model are:
1) Continuously slide a window with size W (e.g., 100ms) along the time series to
extract a group of local segments, with a pref-defined step (e.g., 4ms). 
2) Extract a feature vector from each of the local segments using DWT,
using db3 up to the 3rd level approximation.
3) Similar to the bag-of-visual-words model in images, all local
segments from all time series are clustered by k-means clustering to
create a codebook, i.e, the cluster centers are treated as codewords.
We use a codebook of size 1000, so we run the k-means with 1000 clusters.
4) A local segment is assigned the codeword that has the minimum
distance to the local segment, and the time series is represented as a
histogram of the codewords.
5) The bag-of-words representation is used as input for classification.

With the BOW representation, you trained a one-class SVM using benign traces.


\subsection{Additional Features}
%In addition, we can also add statistical features (e.g., min, max,
%median, std, etc.) and frequency domain features.
 
We plan to add statistics (mean, var, 3rd-nth... momentum) for each
5-sec long window as additional features.
I will compute mean over 5sec window, but will NOT insert that value
into the 100ms window. The purpose for using 100ms window is to
compute (bag-of-phase) features from histogram of phases. The
statistic features are parallel to the bag-of-phase features for the
5sec window. After computing bag-of-phase features for the 5sec
window, I will catenate them with the statistic features together.
}


==> columbia.tex <==
%\begin{figure}[tbp]
%\centering
%\includegraphics[width=0.45\textwidth]{figs/9.columbia/benign-CDF.pdf}\par
%\caption{Columbia CDF}
%\label{fig:columbia-cdf}
%\end{figure}

Our data set is not unique, we obtained a similar data set from ~\cite{perf_counters_2013} and
analyzed it. One of the key things we looked at is the distribution of malware execution lengths. 
For each malware type we summed up all records in the data set
regardless of training/testing partition. Even if the samples
were executed multiple times, we did not distinguish between separate executions because the data set 
~\cite{perf_counters_2013} lacks such information.

As we mentioned before, we did our experiments on the board equipped with ARM A15 CPU
running at up to 2.5GHz
\ref{http://www.arm.com/products/processors/cortex-a/cortex-a15.php}, while the
\cite{perf_counters_2013} ran malware samples on OMAP4460 dev, which is equipped with ARM A9 CPU
running at 1GHz+. Because of using much faster and more advanced CPU, our
average execution times of individual malicious activities shown in ~\ref{} are much lower than
they would have been if we had used OMAP4460 board.  Thus, the
analysis we present here is significantly skewed in the favor of \cite{} data
set. In the \cite{} data set, the time is measured in cycles; when we converted
cycles into seconds, we assumed 1GHz frequency \ref{columbia-cdf}.

When analyzign the distribution of lengths of malicious traces, one can easily notice how short 
they are -- 20\% of malware samples were tested for less
than a second, 56\% - less than 10 sec. We assume that common malicious payload
was not executed in most cases. The total length of all benign traces in
~\cite{perf_counters_2013} data set is 2h 36 min, malicious traces 58 min .
However, the length of all traces in our data set is higher by an order of
magnitude.

Due to space limitation, here we present a brief analysis of 
2 randomly chosen malware samples.
The shortest one is CruseWin coming from the package com.flashp. 
The overall length of all 6 CruseWin’s traces is 0.08138 sec or 
3,061 records. 4 out of 6 traces contain less than 10 records 
each, i.e.  each file spans the execution time of 500,000 
cycles; the rest two files are about 1,500 records. CruseWin 
malware primarily acts as SMS stealer or SMS proxy 
\cite{http://blog.trendmicro.com/trendlabs-security-intelligence/android-malware-acts-as-an-sms-relay/}. 
\cite{HASP} claims that an average phone user has 200-2000 text messages. 
In our experiments, stealing 200 SMS messages took 24 sec, that is 300x 
longer than the length of all CruseWin’s traces in the data set. 

%Second, such small numbers are not appropriate for using 
%statistical techniques used in the paper \cite{perf_counters_2013} 
%to recognize malware.

Even if we look at the malware samples presented by solid 
number of traces, we can notice the same flaw. For example, 
Geinimi malware includes traces 
whose length is only 0.069669 sec or 2631 records. Besides 
stealing SMS, GEINIMI steals contacts, uploads and downloads 
files; each of these malicious actions has time scale of a 
few minutes in our experiments. Hence, the overall length 
of Geinimi’s traces is about 78 sec, but all of them come 
from 18 different packages, thus they are not necessarily 
comparable.

%Other observations:
%The package NickySpy com.nicky.lyyws.xmall is in the malware 
%train set, but it does not exist in the malware test set.

%Total length:

%CruseWin   0.08138 s   100\%

%LoveTrap   0.12082 s   85.7\%

%FakePlayer   0.24879 s   86.7\%

%Zitmo   0.4891 s   100\%

%FakeAngry   0.85992 s   50\%

%NewZitmo   0.91367 s   62.5\%

%DogWars   1.278 s   25\%

%Endofday   1.5679 s   80\%

%Android.Sumzand   1.8054 s   77.8\%

%Tapsnake   2.1969 s   100\%

%Dropdialerab   2.2575 s   81.3\%

%DougaLeaker.A   2.4691 s   62.9\%

%Jifake   3.5979 s   100\%

%AngryBirds-LeNa.C   3.6063 s   79.2\%

%Android.Steek   3.8901 s   100\%

%Loozfon-android   4.5098 s   100\%

%FakeNetflix   4.5393 s   75\%

%KMIN   6.2952 s   83.3\%

%Gone60   7.1543 s   88.1\%

%HippoSMS   9.3769 s   82.1\%

%Bgserv   10.1766 s   85.3\%

%Android.Trojan.Qicsomos   10.4931 s   100\%

%SndApps   14.9489 s   72.7\%

%YZHC   16.6375 s   87.5\%

%GGTracker   23.012 s   60\%

%BASEBRIDGE   27.5132 s   63.8\%

%DroidDreamLight   39.4554 s   82.2\%

%CoinPirate   39.8027 s   70\%

%RogueSPPush   51.563 s   77.6\%

%jSMSHider   55.2832 s   78.7\%

%GEINIMI   78.1776 s   75.9\%

%Zsone   138.1554 s   80.8\%

%Plankton   146.0793 s   78.4\%

%BeanBot   190.6496 s   60.2\%

%PJAPPS   390.4086 s   78.2\%

%GoldDream   745.5366 s   71.3\%

%AnserverBot   1421.8783 s   96.6\%



==> discussion.tex <==
HMDs v. System calls: neither of them sufficient by themselves, but as a part of a
collaborative malware detection system.

QoS and introspection hardware to detect malware. Instead of specialized signatures.

At the hardware level, malware cannot hide.

Wagner and Vern Paxson papers on caution required while evaluating ML for security, specifically anomaly detection.

Fortunately, mobile systems have payload units that can serve as atomic units of 
actions. Might not be the case for some malware.

Real input based runs to seed dynamic analysis + path expander.



==> format.tex <==
%for A4
%\textheight 24.7cm
%\textwidth  16.0cm
\textheight 9in
\textwidth 6.5in
\topmargin 0pt
\topmargin  -12pt
%\headheight 15pt
\headsep    4pt
\baselineskip -1pt
\oddsidemargin 0in
\evensidemargin 0in
%\evensidemargin -14pt
%\oddsidemargin -14pt
\itemindent .05in
\labelwidth .0in

\setlength{\itemsep}{-.5in}
\setlength{\parskip}{\smallskipamount}
\makeatletter
\renewcommand{\section}{\@startsection
  {section}% name
  {1}% level
  {0mm}% indent
  {1pt}% beforeskip
  {1pt}% afterskip
  {\large\bfseries}}
\makeatother


\makeatletter
\renewcommand{\subsection}{\@startsection
  {subsection}% name
  {2}% level
  {0mm}% indent
  {1pt}% beforeskip
  {1pt}% afterskip
  {\bfseries}}
\makeatother


\makeatletter
\renewcommand{\subsubsection}{\@startsection
  {subsubsection}% name
  {3}% level
  {0mm}% indent
  {1pt}% beforeskip
  {1pt}% afterskip
  {\itshape}}
\makeatother

\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> intro.tex <==
Hardware-based malware detectors (HMDs) are a promising new defense against
malicious programs.  An HMD extracts instruction-set and micro-architectural
data from a program's execution, compares this data to a database of benign or
malware executions, and raises an alert when the current execution looks unlike
benign or similar to malware executions.  Recent work in 
%going rapidly from initial proposals 
HMDs uses both off-the-shelf hardware~\cite{perf_counters_2013,anomaly-detector-columbia-raid} and new
hardware accelerators~\cite{map}, and a combination of both techniques
will soon be deployed in commercial mobile devices to augment software-based
malware
detectors.\footnote{https://www.qualcomm.com/products/snapdragon/security/
smart-protect} 

HMDs are valuable as a new line of defense against malware
especially when operating systems get compromised~\cite{master-key,adb-vulnerability,stagefright}, and as a
probe into instruction-set behaviors that are not visible through system calls
or (Android) middleware API calls.  HMDs thus complement traditional
software-level malware detectors~\cite{mihai-issta,fredrikson-near-optimal-specification,kolbitsch-syscall-detection-end-host,apposcopy}. In addition, HMDs 
have a dramatically smaller and 
relatively stable trusted code base than software detectors, and can enable
efficient, always-on malware detection~\cite{qssp,map}. 
These reasons make HMDs extremely attractive to hardware
platform providers like Qualcomm who can collaborate with security vendors like
Symantec and avoid maintaining software-level detectors in sync with upstream
Android distributions.
%can collaborate with malware analysts like Symantec without maintaining an
%entire distribution of Android.  (in collaboration with malware analysts like
%Symantec) without having to maintain an entire distribution of Android.
%dramatically smaller and more stable over time,

Interestingly, evaluating HMDs for mobile malware 
poses new challenges compared to software-based detectors.  
Software detectors look for actions
such as reading contact lists or SMSs---actions that are intrinsic to malware's
goals like stealing private information. 
While sophisticated mimicry attacks can evade
software-level detectors~\cite{wagner-mimicry-attacks},
hardware signals like
instruction-set and micro-architectural behaviors are especially easy to adapt,
by adding multiple threads or delays for example, to create a
diverse set of signals for the exact same goal. 
Thus the first challenge in
evaluating HMDs %and more so than in evaluating software detectors, 
is to account for {\em adaptive} adversaries. 

%Attackers can even attempt to mimic
%benign programs---such mimicry attacks are 
%likely easier against HMDs than software detectors~\cite{wagner-host-ids-mimicry}.
%---prior work on `mimicry attacks' have been shown to circumvent
%software based detectors

%unlike
%system-call or Android API level behaviors like stealing a contact or an SMS 
%that are intrinsic to a malware's goals.  
%the traditional approach of using popular off-the-shelf malware and benign programs. 
%so much so that the HMD's detection results might be meaningless.  
%
%The first challenge is that unlike
%benign programs, malware adapts to evade detector algorithms. 

A further challenge in evaluating HMDs is {\em evasive} malware which leads to
the traditional architecture methodology of using popular, off-the-shelf
programs to produce incorrect results.  Malware, unlike benign programs, is
stealthy and designed to {\em not} execute in emulators and to execute {\em
only} when triggered through specific commands from a remote server.  We find
that off-the-shelf malware binaries~\cite{contagiodump,malware-genome} rarely
execute correctly and show that prior work~\cite{simha-isca} on evaluating HMDs
for mobile malware is unlikely to have triggered malware payloads
(Section~\ref{sec:motivation}). 
%In contrast, we go beyond correct execution and additionally create a
%benchmark

Finally, HMDs perform {\em differential analysis} of benign and malware
execution signals. If benign executions are unlike real program usage or
if the programs receive no inputs at all, malware actions might be the only
(distinctive) executing code and (fallaciously) improve an HMD's detection
rate. 


%HMDs using off-the-shelf malware yields 

%- How robust is an HMD to malware adaptations? range of operation.

%Realizing the potential of HMDs requires new quantitative metrics. 

%in terms of atomic malware actions.
%requires innovations beyond 
%analyzing the behavior of programs at the hardware level, 

In this paper, we present \name---a new methodology to evaluate HMDs that
addresses the above challenges. To account for adaptive and evasive malware, we
deconstruct a large corpus of malware to identify atomic, orthogonal actions
that comprise malware activity. As a result, we can synthesize malware samples
that include the best code and data obfuscation teachniques and whose
hardware-level signals can be tuned precisely. Further, an HMD-generated alert
can be attributed to a specific malware action like stealing contacts or SMSs
instead of being attributed to malware codenames such as Geinimi.a or
AngryBirds-LeNa.C.

To provide the right benign baseline for the HMDs' differential analysis, we
build a new record and replay infrastructure to capture real human interactions
with applications such as a user playing several levels of the Angry Birds game
or fill several forms to diagnose diseases. In Section~\ref{sec:motivation}, we 
demonstrate that real inputs produce considerably different signals compared to
no input or using Android's generic `Monkey' tool to generate inputs. 

%We base our following insights on
%data collected from this rigorous experimental testbed.

%In the process, we also identify that mobile malware
%primarily spreads through user~\cite{permissions,repackaged} or 
%developer~\cite{permissions,advulna} 
%errors instead of 
%traditional exploits such as buffer overflows. Hence, we construct
%a malware benchmark suite 

%against adaptive, evasive malware and differentially analyze
%malware against real user-driven benign applications.
%show that the problem of {\em evaluating HMDs for mobile malware} 
%does not admit traditional benchmarking techniques---
%In response, we
%Based on our tunable malware suite,

Our key insight is a new metric, the {\em operating range}, which quantifies an
HMD's effectiveness. The operating range replaces true positive v. false positive (`ROC') curves for machine learning classifiers used in HMDs.
Instead of ROC curves, an HMD's
operating range shows which malware payloads are detectable for each false
positive rate. The intuition is that since an adversary can generate an
arbitrarily large number of malware signals, an HMD should be rated by the
smallest deviation from benign executions that it can reliably detect. In the
limit cases, even a trivial HMD can detect a malware that is extremely
compute-intensive whereas no HMD should detect a malware which does not execute
a malware action (e.g., a fake AngryBirds just plays the game and doesn't steal
SMSs).
  
\begin{figure*}[tbp]
\begin{minipage}[b]{0.33\linewidth}
%   \begin{flushleft}
   \centering
   \includegraphics[width=\textwidth]{figs/11.motivation/AngryBirds/NEW_AngryBirdsSpace_MOTIVATION.pdf} \\
   Angry Birds game + click fraud 
   \label{fig:motivation-1}
%   \end{flushleft}
\end{minipage}
%\hfill
\begin{minipage}[b]{0.33\linewidth}
%   \begin{flushright}
   \centering
   \includegraphics[width=\textwidth]{figs/11.motivation/Sana_Moca/NEW_MOCA_MOTIVATION.pdf} \\
    Sana medical app + SMS stealer
   \label{fig:motivation-2}
%   \end{flushright}
\end{minipage}
\begin{minipage}[b]{0.33\linewidth}
%   \begin{flushright}
   \includegraphics[width=\textwidth]{figs/11.motivation/TuneInRadio/NEW_RADIO_MOTIVATION.pdf} \\
   Internet radio + password cracker 
   \label{fig:motivation-3}
%   \end{flushright}
\end{minipage}
\caption{
Effect of adaptive malware.
Here, the HMD is trained on `malware-train' input and 
outputs the probability that a given execution matches malware-train (higher is better).
Results indicate a low probability 
of detecting a `malware-test' input that executes the same malicious action with {\em more} threads. 
Worse, the `benign' test input is more likely to be labeled as malware. We conclude that
adaptive malware forces HMDs to model benignware and 
look for anomalies instead of signatures of specific malware executions. 
%Malware can adapt its computational signature to avoid
%malware-signature based detection without reducing its own efficiency. Figures
%show probability of having seen similar execution phases in the malware training set, 
%so lower value implies less likelihood of being labeled as malware. The test malware
%looks even more unlikely to match malware training-set than benign programs.
}
\label{fig:motivation}
\end{figure*}

%Why a malware execution was detected by the HMD? How robust is the HMD to
%variations?

%differential => real benignware, real malware. 
%intelligent malware => 
%   anomaly + threshold

%Insights:
%Payloads, not exploits
%Benign v. Benign'
%Sizes of payloads => tune the machine learning models. simha:25k, Dmitry:10k


%Contributions:
%EMMA
%HMD algorithms: lightweight
%Results: TPs, 

\noindent In summary, our specific contributions include:

\noindent{\bf 1. Rigorous Methodology and New Metric.} We propose to quantify 
the HMDs' operating ranges against adaptive malware and real benignware executions.  
In particular, we determine atomic, orthogonal actions in mobile malware that we
use to create 594 diverse malware binaries and record-and-replay 1--2
hours of real human inputs for each of 9 popular Android applications. 

%\name raises
%alerts not only when a malware is detected but also 

\noindent{\bf 2. Light-weight HMD algorithms.} We use information about atomic malware actions
to extract features and build two light-weight classifiers. For
example, we sample performance counters at 80ms instead of 25k
cycles~\cite{simha-isca}, yet our algorithms are simple to train and can
reliably detect leakage of even a few SMSs or contacts (among other malware
actions) with false positives of 10\%--20\% (equivalent to state-of-the-art in
HMDs for Android~\cite{simha-isca}).  

\noindent{\bf 3. HMDs Composable with Static Analyses.}
We demonstrate that techniques like string encryption and Java reflection
that malware binaries use to evade static analysis tools in turn make malware's
hardware signals more anomalous. This means that HMDs compose well with commercially
deployed (offline) static analyses~\cite{fireeye,lookout,avast,evade-bouncer,flowdroid}.


While the \name approach 
%of measuring operating ranges of detectors against adaptive malware 
is applicable to evaluating both hardware and software based
malware detectors, 
%against intelligent adversaries, 
this paper specifically focuses on diversifying hardware signals and evaluating
the operating range of hardware-based detectors only.  We will release \name,
including real and diversified malware binaries, tools to record and replay
user traces, code to instrument Android devices, our HMD implementations, and
our entire user input and performance counter dataset, to researchers upon
request.\footnote{EMMA has been used at Qualcomm and shared 
with a university research group.} HMDs form an exciting
new research area for computer architects, and the \name methodology and platform
lay a sound methodological foundation for future research in this area.





%As a result, there has been considerable
%research into creating HMDs based on existing hardware performance
%counters~\cite{simha-isca13,simha-raid-14} and new hardware
%probes~\cite{cchunter}, implemented as hardware accelerators~\cite{hpca-dmitry},
%and even deployed in a commercial product~\footnote{sphinx}.  


%HMDs' most significant value
%lies in their small trusted code base -- millions of lines of code
%in the operating system and middleware need no longer be trusted -- 
%and in being able to observe instruction-level program 









\ignore{

Behavioral analysis is an important line of defense against malware.
%Behavioral malware detectors are classifiers built using 
%
Using behavioral signals such as 
%events~\cite{sql-inspection}, 
system calls~\cite{mihai-issta} and network traffic~\cite{bro-snort}, 
%from benign and malicious programs 
an analyst can train a malware detector and then use it to label program
executions as benign or malicious.
%can be used as behaviors to build classifiers with.  that are used to label
%program executions at run-time as either benign or malicious.  
%
Similarly, hardware behaviors -- assembly instructions, memory access patterns,
branch mispredictions, etc -- have also been proposed to train malware
detectors.  Such hardware-based malware detectors (HMDs) are particularly
compelling because of their ability to
%present a small trusted code base, and hence can potentially
expose malware even if applications or the kernel are
compromised~\cite{user-error-permissions,master-key,ad-vulna}. 

\mohit{if a malware functionality didnt execute, is the execution malicious?}
\mohit{HMDs can be split into hardware signals and hardware accelerators for
machine learning/classifiers}

An appropriate evaluation methodology is crucial to unlocking the
potential of HMDs. 
HMDs lack access to application-level semantics resulting in
missing malware
(i.e. low true positives) as well as misclassifying benign applications (i.e. high false
positives).
%On the other hand 
In contrast, software-level detectors can check for policies such as `an app
should access only one, and the most recent, SMS', or `an app can access
medical records only after two-factor authentication'.
%
%Hardware signals performance counter or dynamic instruction traces do do not
%carry information about 
It is not obvious that such application-level access control policies will be
discernable by HMDs. 
For example, can instruction mixes 
or load-store patterns expose malware such as click fraud in a web-browsing app?
%result in a 
%detectable signal?
%for example, or that click
%fraud in a browser will have a measurably distinct load-store behavior.
%and as a result hardware detectors may miss malware or raise false alarms.
%Given their benefits and challenges,  correct and appropriate
%determine the feasibility of hardware-based malware detectors. 

%We compared 20 malware (from UCSB security lab dataset) vs. 20 benignware
%(e.g., pdfviewer, calculator, filetransfer, resizer, screensaver) on Windows. 
%
%In summary, Windows malware executed ~60K syscalls within 10 minutes v. only
%2.5K for benignware. RegSetValue, the system call used to modify Win registry,
%is invoked 820 times by malware and only 72 times by benignware on average.
%Further, malware spawns 182 processes/threads on average (outliers: virut -
%364, kuk - 335), while benignware spawns fewer than 30.
%
%For our Android dataset, there is no statistically significant difference
%between malicious and benign apps’ syscalls: our detector thus looks for
%anomalous phases.
%

This paper focuses on evaluating HMDs for mobile malware.  Mobile malware is
typically hidden in benign applications (``parent'' apps), and abuses user-level
access control permissions to execute their payload.  Most mobile malware does
not rely on traditional exploits such as buffer overflows, SQL
injection, etc. to escalate privileges.
%that are driven by user, network, and sensor inputs. 
%Our experiments show that 
In contrast to mobile malware, 
traditional desktop malware leave a distinct system call footprint.
This footprint is evident due to changes to the Windows registry
as well as the launch of several child processes.
%In contast, mobile malware typically 
Can machine learning classifiers designed for desktop malware be tuned to work
with hardware signals instead?
%Will hardware signals expose an `SMS-trojan' that messages premium-rate
%numbers by hiding within a legitimate messaging app?  

%present unique challenges to computer architects' quantitative approach to
%evaluating systems
%
%Specifically, we propose a  

To answer such questions rigorously, we designed and built 
\name\footnote{``the cosmic illusion that the phenomenal world is real'' http://www.britannica.com/EBchecked/topic/370816/maya} :  
%a system that provides malware and benignware programs a
a realistic, controlled environment to record and replay both
malware and their parent benignware,
along with a set of machine learning classifiers as the HMDs under test.  
%Our key contribution is an HMD evaluation methodology 
\name is built around two novel principles: 
%-- the threat of an intelligent adversary, who knows the proposed HMD and
%actively obfuscates the measured hardware signal, and the problem of creating
%appropriate benign executions to contrast malicious ones with.
% 
%We posit that 
~\\ \noindent{\bf Intelligent adversary.} First, unlike benchmarks such as SPEC
or Parsec, malware is written by adversaries who will adapt malicious
computations in response to a deployed HMD. For example, by adding threads or
delays to the computation, by changing the binary that implements an
application-level behavior, or by reordering the sequence of malicious events,
a developer can dramatically alter the hardware signal while retaining the
malware's high-level behavior. 
To account for such adaptive malware, 
we created a diverse population of malware and
benignware programs and use these to evaluate HMDs.
%computations to obfuscate their hardware signals.  Instead, off-the-shelf
%mobile malware samples that were written for a system without HMDs attempt to
%be as efficient as possible while evading currently deployed defenses like
%static analyses~\cite{isil-malware} and emulator based dynamic
%analyses~\cite{taintdroid,google-bouncer}.  to actively obfuscate the hardware
%signals being measured only serves to build false (and temporary) confidence
%in the HMD.
%

\noindent{\bf Appropriate benign executions.} Second,
%
%Simply launching a mobile application puts its main activity in a loop waiting
%for user input, and comparing malware signals to this baseline `silence' will
%yield incorrect detection and false positive rates. Instead, 
we propose that malware execution signals should be compared against {\em its
parent application's signals} instead of signals from an arbitrary benign
program. For example, a malware like Geinimi should be compared against
its parent, the MonkeyJump game, instead of an arbitrary program like {\tt/bin/sh}.  Further,
the benign application signals should reflect {\em real computation} -- i.e.,
respond to user inputs, redraw the screen, execute all background services, and
have its computational intensity impacted by network- and system-level noise.
Without real inputs, comparing malware signals to signals from a dormant
application will yield incorrect detection and false positive rates.
%
%Further, malware computation will be interleaved with the parent's benign
%computation. Hence, comparing a malware trace from Geinimi.a with an arbitrary
%program like {\tt /bin/sh} instead of plain MonkeyJump will yield
%unrepresentative detection rates. 
%
%In summary, treating HMDs like SPEC benchmarks is not sufficient -- HMDs have
%unique aspects that require a novel quantitative approach for their
%evaluation.



%
%The malware population includes carefully {\em diversified and obfuscated
%malware} payloads,  while the parent-benignware population covers nine popular
%and diverse applications. We recorded 1--2 hours of {\em real user inputs} to
%drive each parent application; for example, playing games like AngryBirds or
%Zombie World War, or completing medical diagnostic questionnaires in a medical
%app from MIT (Sana).  We built a record-and-replay infrastructure to compare
%malware v. its parent-benignware's signals {\em generated from the same
%user-input} 
%%this ensures a true apples-to-apples comparison 
%on real hardware devices. 

Based on these two principles, we propose a new metric for evaluating HMDs.
HMD evaluations should attempt to 
%`benign parent-app v. malware payload' matrix in addition to true positive v.
%false positive curves~\cite{simha-isca,raid,hpca}. The goal of this result
%matrix is to 
determine the {\bf detection threshold} of an \\
HMD, i.e., the payload whose
hardware signals are distinct enough to be reliably classified as malware.
Detection threshold is a better metric than true positives. To see why,
consider a malware execution where the payload didn't execute -- this trace
should {\em not} be classified as malware by a dynamic program analysis (here,
the HMD). In contrast, a malware payload that steals 10GB of data (for example)
will almost surely be detected as malware.  Since the adversary will attempt to
stay undetected, we can assume that she will pick a payload that stays just
below the detection threshold.  Hence, the goal of an HMD evaluation should be
to find the tipping point -- the malware payload settings where the HMD becomes
reliable at classifying malware from its parent benignware.  The \name approach
is thus a radical departure from testing old, static malware against an
unrelated benign program. 
%without equalizing the user-inputs to both programs.

%is more reasonable than reporting a true-positive number from a 
%crosses over from low/unreliable detection to high/reliable detection is 
%Since the choice of the
%malware benchmark suite directly affects the true positive percentage -- which
%then means little since the intelligent adversary can change malware
%computations -- it stands to reason that identifying the detection threshold is
%a more appropriate measure of an HMD.

%The scale and fidelity of the \name is significantly greater than prior
%work that used off-the-shelf malware

Our specific contributions include:
\begin{description}

%\item We analyzed 72 actual mobile malware families to construct a taxonomy of
%abstract behaviors -- classifying these into tasks such as stealing
%information, conducting network-based attacks, or computational tasks. 
%%
%We then generate a suite of 66 malware payloads whose concrete computations are
%obfuscated and tuned to have less, more, and highly distinct hardware signals.
%We then inject the payloads into our benchmark suite of 9 parent apps. 
%%
%Since the abstract tasks of malware remain constant, 
%%our malware generator outputs 
%the 66$\times$9 malware binaries' executions can be compared to the 9 benign
%apps' traces.

\item{\bf Representative Malware.} 
%We propose a new methodology for evaluating mobile malware.
\ignore{Taxonomy -> Rep malware -> adaptation.} 
%We present a taxonomy of current
%mobile malware payloads based on a manual analysis of 175 malware samples
%(belonging to 72 malware families from 2012-13). 
We classify malware functionality
into {\em information stealers}, {\em network \\nodes}, and {\em
computational nodes}, 
and design a malware benchmark suite based on real malware
binaries for each behavior.  We reverse-engineer the real binaries, 
and complete their server-side functionality to  
ensure that they successfully execute payloads such as stealing data.
We use these real samples to seed a suite of 66 {\em synthetic} malware binaries
%allows an analyst to choose behaviors, specify detailed parameters for each
%behavior, select obfuscation techniques and a baseline application to
%repackage the payload into, and automatically
%that incorporates the best obfuscation techniques 
with a diverse computation profile.
%yield a computationally diverse set of 66 payloads. 
%chosen specifically to
%expose a detector's breaking-point.  
We then inject these 66 payloads into {\em each} of 9 popular
and computationally diverse benign applications, yielding a total of
594 distinct malware binaries.  This malware
benchmark suite is representative, executes correctly, and 
can help identify an HMD's detection threshold.
(Section~\ref{sec:malware-gen}).

\item{\bf Real user-driven execution.} 
We 
%select {\em nine popular and diverse baseline applications} and 
{\em record} real users driving each application through 5--12 minute sessions, such
as completing six medical diagnostic forms, playing seven levels of Angry Birds,
listening to internet radio and switching channels, etc., to generate
user-input traces 56 to 111 minutes long across 9 benign apps.  We then replay
these user-inputs with each benign app contributing 7--10 sessions to the
training set and 2--3 sessions $\times$ 66 malware samples to the testing
set. \mohit{Only report total testing v. training time?}  
We populate two Android development boards with realistic data like SMSs,
photos, etc. in each device 
and extract performance counter traces for all executions (Section~\ref{sec:impl}).
%Overall, \name represents a significant jump in evaluation fidelity over prior
%work~\cite{demme-counters} where over 50\% of the traces (from malware like
%{\tt CruseWin} and {\tt AngryBirds-LeNa.C}) are
%shorter than 10s and are compared to benign apps like 
%{\tt /bin/sh}, {\tt BubbleShooter} etc.

%a novel methodology to evaluate HMDs, a new workload for 
%computer architects.


\item{\bf Anomaly detection HMD algorithms.}
%We propose an alternate approach of constructing signatures of benign apps and
%detecting malware as {\em computational anomalies}.
%
We present two qualitatively distinct HMD classification algorithms -- a
probabilistic Markov model and a statistical bag-of-words model.  Both
algorithms (intuitively) model benign apps as a sequence of program phases.
While the Markov model explicitly captures state transitions over time, the
bag-of-words model only learns the distribution of words (phases) in a document
(a larger time window). 
%The intuition in both cases is to model benign apps as a set of distinct,
%repeating program phases.  (and phase transitions for the Markov model). 
%
Both these models are considerably simpler to train than hidden markov models
or neural networks, and serve as a baseline for potential research into more
complex models (Section~\ref{sec:arch}).
%that are much more complex to train.  we extract features using Discrete
%Wavelet transform, and then creating 
%
%Our experiments with executing malware payloads to completion reveal that
%malware payloads can last several seconds. 
%

%without affecting
%detection rates adversely. 

\item{\bf Malware Detection Results.}
%We achieve good detection rates for several malware-app combinations.  
Surprisingly, even a small payload such as stealing tens of photos, SMSs, or
contacts detectably alters the compute signature of a complex app like Angry
Birds.  User-driven apps like Sana\footnote{A medical diagnostics app:
http://sana.mit.edu/}, or network-driven apps like TuneIn Radio are even more
detector-friendly.
%
However, since very small payloads
such as stealing device IDs are not detected, we conclude that malware can
still escape, but by lowering its payload's performance.
%
False-positive rates for 30 seconds to 1 minute of benign app usage is close to
7\%, motivating further research into integrating HMDs with
carefully chosen software-level signals. 
%which indicates that hardware detectors will have to be 
%a trigger for deeper program analyses.
%OS/emulator-based forensics instead of stand-alone
%detection.  


\name's realism uncovers simpler HMDs that use longer phase durations
(80ms--100ms) and slower sampling rate (per 1ms v. per 25K cycles between two
performance counter snapshots) work better in comparison to prior
work~\cite{demme-counters} (to detect malware with similar goals). 
Interestingly, we find that Markov model and bag-of-words models are 
complementary and a complex app like AngryBirds is better modeled with the
{\em simpler} bag-of-words technique.
Finally, we find that techniques  
%to obfuscate code from static analyses
like reflection and encryption that thwart static analyses in turn make
malwares' hardware-level traces {\em more} anomalous. This means 
HMDs compose well with commercially deployed (offline) static analyses.

\end{description}







%%%%%%%%%%%%%%%%%%%%%  Graveyard  %%%%%%%%%%%%%%%%%%%
\ignore{

\mohit{
* RISC style positioning: quantifying malware behavior 

}


%Mobile malware is a major and growing problem -- estimated size and significant
%growth. \todo{fill this}. 

Mobile malware is an important and growing problem~\cite{kaspersky-report,
risk-iq, cisco, trend-micro-2013-14}. Of the 1M or so applications (or
``apps'') in the official Google Play store, 42,000 were classified as malware
in 2013 -- up from 10,000 of 0.4M apps in 2011~\cite{risk-iq}.  
%Third-party app stores contain even more malware. Trendicro has reported
%detecting 1.3M unique samples of malware across all third-party app stores in
%2013~\cite{trend-micro-2013-14}.  Users looking for free or discontinued
%versions of popular applications often end up with the application repackaged
%with a malicious payload. Although Google uses tools such as
%Bouncer~\cite{bouncer} and Verify~\cite{google-verify} to analyze apps,
%researchers have shown that these tools can be evaded relatively
%easily~\cite{evade-bouncer}.
%
Offline analyses to detect mobile malware are well established, and include
signed binaries~\cite{android-sign}, monitoring use of sensitive
permissions~\cite{android-demystified}, and static~\cite{ernst-taint-type,apposcopy} and
dynamic~\cite{taintdroid,dynodroid} program analyses.  
%
However, these offline techniques do not protect users from attacks on deployed
devices~\cite{ad-vulna,webview-attacks,evernote,applocker,user-error-permissions,RAT,master-key,anomaly-detector-columbia-raid},
therefore leading to recent proposals for 
%there is a pressing need for effective 
{\em online} detectors~\cite{perf_counters_2013}. 
%
 
Specifically, {\em hardware}-based online detectors have valuable attributes such as
visibility into all software level action even with a compromised OS, and a
small, slow-to-change trusted code base (compared to the Android system, for
example).  These detectors use signals such as hardware performance counters to create 
%-- using machine learning or signal processing techniques -- models of benign
%and/or malicious applications (`apps') As a result, hardware-based detectors
%have been used to recognize 
mobile malware signatures~\cite{demme-counters} and to identify desktop malware as
computational anomalies~\cite{anomaly-detector-columbia-raid}. If deployed with hardware
support~\cite{map}, hardware-based detectors promise energy-efficient, online
malware detection. 

However, existing hardware-level detectors have a major handicap -- they lack access to
app-level semantics which can lead to false positives and negatives.  On the other hand 
an Android-middleware level detectors can enforce policies such as `an
app should access only the most recent SMS and do so only for two-factor
authentication'.  Hardware performance counter or dynamic instruction traces do
not have such semantic information and as a result hardware detectors may miss malware or raise
false alarms.  Given their benefits and challenges,  correct and appropriate
evaluation is crucial to determine the feasibility of hardware-based malware detectors. 
%have to be evaluated.

In this paper, we present \name -- a novel methodology to evaluate the detection
performance of mobile malware detectors.
%Our key insight is to 
\name is a significant departure
from prior evaluation methods~\cite{perf_counters_2013} that take off-the-shelf malware
binaries, do not ensure correct payload execution, and compare malware to
arbitrary benign programs that are not driven by real user-input. In contrast, 
\name is based on four principles: (1) malware binaries should execute {\em correctly}
during experiments, even if the binaries have to be altered to do so 
(Figure~\ref{fig:geinimi-crash}); (2)
evaluation should aim to find out {\em why} a detector fails when it does so,
%adaptive malware, 
i.e., instead of true positive percentage, the goal is to
identify the largest malware payload that evades detection; (3) false positive
rate should be determined by comparing malware to its {\em most closely related} benignware
instead of arbitrary apps (Figure~\ref{fig:pca_benign_repack}), and (4) all app executions should be driven using
real user-inputs, else the comparison between dynamic executions of malware and benign apps
is not appropriate.  

\ignore{\todo{To evaluate \name ...}} To demonstrate how malware analysts can use \name,
we present two algorithms for hardware-based {\em anomaly-detection} of mobile
malware.  Anomaly detectors~\cite{classic-anomaly} model traces from only
benign executions and label (in our case, hardware computation based) anomalies
as malware.  We 
%(and concurrent work on detecting exploits on desktops~\cite{raid}) 
choose anomaly-detection in order to detect new or unknown mobile malware.
Previous {\em signature-based} hardware detectors are
limited to detecting {\em known} malware~\cite{demme-counters},
while previous anomaly detectors~\cite{anomaly-detector-columbia-raid} do not detect
{\em mobile} malware.
%We observe that changing the number of threads in a malware payload
%dramatically alters its performance counter signature.  while previous anomaly
%detectors do not target {\em mobile}
%malware~\cite{anomaly-detector-columbia-raid}.  an anomaly detector since the
%alternative approach -- a {\em signature-based} detector trained on {\em both}
%malware and benignware~\cite{demme} -- is best suited to detect {\em known}
%malware.  However, new malware can adapt their hardware-level signatures while
%benign apps do not actively try to evade being modeled.   A new malware binary
%generated by While benign apps do not deliberately evade being modeled, 
However, whether a hardware-based anomaly detector can capture benign executions of mobile
apps -- that comprise of Java, native, and HTML/js components, complex Android
middleware, and driven by real users through rich gestural interfaces -- well
enough to have low false positives is an open question.
%-- for reference, Symantec aims for no more than 0.1\% false
%positives~\cite{symantec-fp}.  Hardware-based anomaly detectors have been
%evaluated to detect desktop malware exploit kits in a concurrent
%project~\cite{raid}. Our platform is specific to mobile malware -- evaluating
%payloads as opposed to exploits (Section~\ref{sec:malware}), comparing to apps
%that include . 

%As such, our anomaly detector is complementary
%to existing malware-signature detectors~\cite{demme} 
%and superficially similar
%to desktop-based anomaly detectors~\cite{raid}. 
%The advantage of detecting previously unknown malware. 

%We justify these
%three principles before describing our specific contributions below.

To answer this question quantitatively, we make the following specific
contributions:
%that benign apps do not try to actively evade being modeled and {\em
%real-world} 
%the anomaly detectors using a large dataset generated from real user-driven
%executions. Our benign dataset includes 9 diverse apps driven by real users

\ignore{\todo{ 1-2 Hours of benign and 594 malware samples hidden in 6000 minutes of
benign execution.}}



%and
%aims to characterize the operating range detector

%has serious implications for future research in this exciting research area.

%{\bf Hardware-based Detector Overview.}
%Building models offline. Detecting online.
%Similar to spam detectors.


%\noindent {\bf Contributions.} 
%We make the following specific contributions to address these challenges and
%prototype \name:

\noindent{\bf 1. Representative Malware.} 
%We propose a new methodology for evaluating mobile malware.
\ignore{Taxonomy -> Rep malware -> adaptation.} 
%We present a taxonomy of current
%mobile malware payloads based on a manual analysis of 175 malware samples
%(belonging to 72 malware families from 2012-13). 
We classify malware functionality
into {\em information stealers}, {\em network nodes}, and {\em
computational nodes}, 
and design a malware benchmark suite based on real malware
binaries for each behavior.  We reverse-engineer the real binaries, 
fix them to work correctly, and complete their C\&C server functionality. 
We use these samples to build a suite of 66 {\em synthetic} malware binaries
%allows an analyst to choose behaviors, specify detailed parameters for each
%behavior, select obfuscation techniques and a baseline application to
%repackage the payload into, and automatically
%that incorporates the best obfuscation techniques 
with a diverse computation profile.
%yield a computationally diverse set of 66 payloads. 
%chosen specifically to
%expose a detector's breaking-point.  
We then inject these 66 payloads into {\em each} of 9 popular
and computationally diverse benign applications, yielding a total of
594 distinct malware binaries.  This malware
benchmark suite is representative, executes correctly, and 
can help identify a detector's breaking-even point -- principles
1 and 2. (Section~\ref{sec:malware-gen}).
%set of 66 malware samples chosen so as to identify a detector's
%breaking-point.

%\todo{WHy -> tune detector to as light as possible -> break-even
%Diverse apps -> real inputs -> replay
%Two ML algorithms.}
%-----------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/geinimi-crash-ind_branch.pdf}\par
   \caption{Executing malware correctly: The off-the-shelf Geinimi.a malware 
causes the underlying app to crash immediately. 
The fixed version is able to carry out malicious actions such as stealing
SMSs or contact information --  we propose to use fixed malware samples to
evaluate detectors.}
\label{fig:geinimi-crash}
\end{figure}
%-----------------


\noindent{\bf 2. Real user-driven execution.} 
Principles 3 and 4 require benign apps to be executed by real users
and then {\em replayed} with the same user inputs but this time with
malware executing concurrently. To this end,
we 
%select {\em nine popular and diverse baseline applications} and 
{\em record} real users driving each application through 5--12 minute sessions such
as filling six medical diagnostic forms, playing seven levels of Angry Birds,
listening to internet radio and switching channels, etc., to generate
user-input traces 56 to 111 minutes long across 9 benign apps.  We then replay
these user-inputs with each benign app contributing 7--10 sessions to the
training set and (2--3 sessions $\times$ 66 malware samples) to the testing
set.  We populate two Android development boards with realistic data like SMSs,
photos, etc and extract performance counter traces for all executions.
Overall, \name represents a significant jump in evaluation fidelity over prior
work~\cite{demme-counters} where over 50\% of the traces (from malware like
{\tt CruseWin} and {\tt AngryBirds-LeNa.C}) are
shorter than 10s and are compared to benign apps like 
{\tt /bin/sh}, {\tt BubbleShooter} etc.

%\ignore{Overall,
%our experiments generate training sets of almost 40 to 90 minutes across the 9
%benign apps and tested against malware hidden in 300 to 600 minutes of app
%usage.  \todo{check durations.}}


\noindent{\bf 3. Anomaly detector algorithms.}
%We propose an alternate approach of constructing signatures of benign apps and
%detecting malware as {\em computational anomalies}.
%
We present two models -- a temporal, probabilistic Markov model and a simpler,
statistical bag-of-words model (that uses one-class SVMs).  The intuition in
both cases is to model benign apps as a set of distinct, repeating 
program phases (and optionally, phase transitions). Both these models are considerably simpler to
train than hidden markov models or neural networks and serve as a baseline for
potential research into more complex models.
%that are much more complex to train.  we extract features using Discrete
%Wavelet transform, and then creating 
Our experiments with executing malware payloads to completion reveal that payloads can
last several seconds. This enables
 simpler models, longer phase
durations (80ms--100ms), and low-frequency performance counters sampling 
(per 1ms v. per 25K cycles) v. prior work~\cite{demme-counters} 
without affecting detection rates. 

%such that many atomic actions in
%malware payloads are longer than this phase duration and cause a detectable
%anomaly at runtime.
%sampling rate is low based on characterizing mobile malware payloads


\noindent {\bf 4. Detection Results.}
%We achieve good detection rates for several malware-app combinations.  
Surprisingly, even a small payload
such as stealing tens of photos, SMSs, or even contacts in a batch detectably
alters the compute signature of a complex, computationally intense app like Angry Birds. 
User-driven
apps like Sana\footnote{A medical diagnostics app: http://sana.mit.edu/} 
or network-driven apps like TuneIn Radio are {\em even more}
detector-friendly.
%
Since very small payloads
such as stealing device IDs are not detected, we conclude that malware can
still escape, but by lowering its payload's performance.
%
False-positive rates for 30 seconds to 1 minute of benign app usage is close to
7\%, motivating their use as 
%which indicates that hardware detectors will have to be 
a trigger for deeper OS/emulator-based forensics instead of stand-alone
detection.  
%
Interestingly, we find that Markov model and bag-of-words models are 
complementary and a complex app like AngryBirds is better modeled with the
{\em simpler} bag-of-words technique.
Finally, we find that techniques  
%to obfuscate code from static analyses
like reflection and encryption that thwart static analyses in turn make
malwares' hardware-level traces {\em more} anomalous. This means 
hardware detectors compose well with commercially deployed (offline) static analyses.
%Further, for AngryBirds, a simpler statistical model yields better 
%detection rates since by accounting for phase transitions, the Markov model
%becomes worse.
%MM and BoW are complementary.
%-----------------
\begin{figure}[tbp]
\centering
\includegraphics[width=0.34\textwidth]{figs/pca-benign-vs-repackaged-vs-random-apps_combined.pdf}\par
\caption{Comparing malware to the closest benign app.
The plot shows principal components of benign Firefox's traces, 
traces from Firefox infected with malware, 
and the traces of randomly chosen Android apps. 
Infected Firefox's traces are closer to baseline Firefox than to random apps.}
\label{fig:pca_benign_repack}
\end{figure}
%-----------------




%\ignore{1. True positives:real.  where is the break even point.
%2. False positives?
%3. Encryption.
%4. Different board?
%}
\ignore{\todo{downsampling, less counters.}}

In summary, \name enables research into hardware based malware detection by
providing a platform for correct and consistent execution of representative
malware samples.%\ignore{transition to motivation?}

\ignore{
\name's prototype enables large-scale analytics on hardware signals.
Our prototype builds models of benign apps being driven by real users
for 1--2 hours 
helps uncover several insights that are.

The dearth of semantic information is a major handicap for
hardware-based detectors.  
%For example, a hardware level detector cannot
An app may have permissions to access SMSs to ease two-factor
authentication or to Contacts for in-app messaging, but when compromised 
the app may access all SMSs/Contacts in sequence
and exfiltrate them. Software-level detectors attempt to prevent such
malware using contextual policies such as `all SMS/Contacts accesses 
must be authorized through a trusted user-interface'~\cite{dawn-contextual,apposcopy}.
Can hardware detectors identify malware
that exercises very similar behavior as benignware but for malicious ends?

%hardware detectors do not have access to such semantics and may miss 
%malware (`false negatives').

Further, without app-level semantics, {\em false positives} may be 
a major hurdle for behavioral detectors to be
deployed in the field, with Symantec targeting to keep false positives below
0.1\%~\cite{symantec-fp}. 
%a user may accidentally visit a compromised website that uses the native  
%%which URLs an {\tt iframe} is allowed to access or 
%such as which SMSs an app has legitimate access to (i.e. an app with
%SMS access permissions may be malicious and exfiltrate private SMSs undetected)
%Mobile apps are complex and comprise of event-driven services written in managed,
%native, and web-based languages that interact with platform services and that 
%include several third-party libraries for analytics, advertising, etc.
%(Java, Objective C), native (C/C++/asm), and web-based (javascript/HTML) languages.
%A large part of functionality is implemented through platform services 
Consider AngryBirds -- an app that includes Java and web-based components to implement
a gesture-driven user interface, native components for the game engine and rendering, and
libraries for analytics, advertising, and in-app payments.
%Mobile apps comprise of complex functionality written in managed, native, and web-based
%languages with very diverse user interactions including .
A new hardware-level 
behavior might be triggered by the user unlocking a new functionality in an
app (e.g. a level in a game). Or, contention for hardware and platform
services (such as SMS database) from other
apps may alter the app's hardware execution profile.
Will a hardware detector simply flood users with false malware warnings?

%Given the diversity of hardware level behavior of both benignware and
%malware, 
%is another challenge that worsens detection rates and false positives.
%Given these opportunities and challenges, 
%{\em evaluating} hardware detectors
%appropriately is critical to quantify their expected in-field detection rates. 

%, with the growing interest in malware detectors, requires an
%appropriate .

% such as hardware performance counters contain
%information about app executions' dynamic instruction stream and
%micro-architectural behavior, and have been evaluated as a detector for
%malware-signatures~\cite{demme} (for mobile apps) and
%malware-as-anomalies~\cite{raid} (on a desktop browser and PDF reader).
%Hardware accelerators to detect malware~\cite{hpca-map} have also been 
%proposed to recognize malware-signatures at run-time.

%With false positive rates of \todo{$\sim$20\%} for a true positive rate of
%\todo{$\sim$80\%} hardware-based detectors seem to be promising candidates for
%light-weight, on-device filters that can trigger more detailed dynamic analyses
%(based on record and replay~\cite{} and deep packet inspection~\cite{} for
%example).


%Evaluating hardware based detectors under {\em realistic} conditions, however,
%remains a major concern.
%
%On the one hand, hardware-based detectors have the advantage that instruction
%sets and performance counter interfaces are simpler, change slowly (compared to
%Android's API for example), and can observe malware activity even if the OS is
%compromised by `rootkits'~\cite{rootkits}. 
%


%%
%While prior work evaluated detectors using off-the-shelf 
%malware datasets, 

%Given the diversity in legal programs and the volume of data,
%{\em evaluating} hardware-based malware detectors is a challenging problem.
%The challenges are compounded further malware samples available online 
 
We find that {\em evaluating the malware detectors themselves} 
poses unique challenges that do not arise in traditional
program-phase analyses~\cite{phase} that hardware detectors are inspired by.

Similar to the case for managed language benchmark suite 
(by Blackburn et al~\cite{smell-coffee}), establishing a {\em representative}
and {\em realistic} evaluation methodology is foundational for 

Rigorously quantifying the potential of hardware based malware detectors poses
several open questions.
- did payload execute correctly?
- compare to benign?
- why did a payload get detected?
- can a malware avoid detection, or in other words, how robust is the detector?

%even if they are to even serve as a first level filter that trigger more
%detailed program~\cite{} or manual analyses~\cite{}.


%In this paper, we propose a new methodology for evaluating hardware-based 
%mobile malware detectors. 


%What makes mobile malware different from desktop variants?
%Challenges and opportunities.

%Yet surprisingly little is understood about what the malware is attempting to 
}


}

}



==> malware_classification.tex <==
We started from the analysis of existing Android malware and discovering the global trend on mobile malware market. Also, we wanted to analyze how Android malware has evolved since the time ~\cite{dissect_malware_2012} was published. As opposed to ~\cite{dissect_malware_2012}, our goal was not to completely characterize all types of Android malware, instead we focused on characterization of the most widespread malicious programs. In the following experiments, we used publicly available malware samples downloaded from ~\cite{contagiodump}, ~\cite{malware.lu} and ~\cite{virusshare.com}.

Our main interest was to classify dynamoc behavior of malicious software. Deep understanding of dynamic behavior provides opportunities for its effective real-time detection, and also eliminates issues related to the use of static methods such as static signature.

At the highlevel we assigned every malicious payload to a few of the following three categories: information stealers, network nodes, computational nodes. Information stealers are looking for the sensitive data and uploads it to the server. A mobile device contains lots of private data, and it is designed to grant its owner an easy access to the private data. We distinguished two types of sensitive data: user-specific and device-specific. Sensitive user-specific data incorporates large variety of different data types, including - but not limited to - contacts, emails, text messages, photos, apps information. Sensitive device-specific data is mainly represented by device identifiers - IMEI, IMSI, ISDN. The second category of malicious apps in our highlevel classification utilizes a mobile device as a network node. It means that malware uses a device to access the Internet resources. In this case the concrete physical device has little value; what is really important is the network bandwith. And finally the last category of malware may carry out distributed computations on mobile devices. We have not observed such a malware, however we expect that it will emerge in the future.

After identifying a highlevel structure of malicious applications, we digged deeper in order to understand the underlying black market model. Not only technical flaws create favorable conditions to prosper, but also under-regulated legal environment. We pose a question why people collect someone else's personal data, because we wanted estimate how important information stealing in mobile world is and will be in the future. It turns out that numerous malware models have been deployed that cover the whole range of use cases, from completely illegal zone to the "grey" one. There exist many mobile applications that spy on a person or group of people. Some companies officially sell such a spyware, for example, ~\cite{copy9}. Later such an information could be used to compromise smartphone owners. Other apps may collect personal information to better serve their users i.e. to learn their preferences, or for marketing purposes. On the other hand, stealing sensitive device-specific ids does not affect the privacy of real people. On the black market, stolen device IDs are used to legalize stolen physical mobile devices. A network provider may ban a device with a particular ID to connect to the cell network after receieng a report that a device has been stolen. However, criminals replace IDs of a stolen device with IDs of a legitimate device that can be bought on the black market.

We have noticed a trend towards the more intensive usage of devices as network nodes. Two years ago, the authors of ~\cite{survey_malware_2011} claimed that mobile phones present challenges for DDoS attackers because of low bandwith and low battareis cappacity. Since that time, network bandwith has improved substantially and becme comparable to desktops bandwith. We noticed a few modest attempts to build a DDoS attackers, however, nowadays DDoS'ing webresources with mobile devices are not popular at all, and we think that there are might be economical rather than technical reasons for that. 

Usage of mobile devices as a network nodes seems to be at least as much profitable as stealing personal information. Ad clickers, the apps that click on a specific web links, prevails in this category. There are also "gray" programs that downloads some files including other apps in order to raise tha ranking of a malicious resource or a particular malicious app even in an official app store. We have not observed malicious applications that offload computations to mobile devices, but we expect that such applications will emerge when mobile devices' batteries improve. The analysis of the black market economic model shows that the demand in malicious software is growing, and it will not decrease in the near future. In other words, it motivates us to focus on protection of mobile systems against malware types mentioned before.

The common thing of most existing malicious applications on Android platform is that they heavily rely on social engineering techniques. Usually, they do not use complex kernel exploits or flaws in Android middleware. Developers of malicious programs include them into a benign applications, especially into paid apps, and distribute on a 3rd party markets for free. This method is called "repackaging" in the classification presented in ~\cite{dissect_malware_2012}. One more popular method of distributing Android malware is to create so-called "renamed" apps: a fully malicious app uses a name of a legitimate app. When a user installs such an app, it quickly executes its malicious payoad, shows an error message to pretend to be a legitimate app and quits.

After identification of most prevalent malicious behaviors, we created a tool that can model both malware existing in the wild and far more advanced malware samples that we have not observed so far. Our framework helps us to study the limits of our approach to malware detection. Modeling of malicious behavior is achieved by injecting malicious payload into a benign Android application. The injected malware incorporates all previously discussed types of the existing malware and adds multiple delays to control intensity of malicious behavior. We also model command and control server (C\&C server) that guide malware execution.

We treat each malware subcategory as a {\it malware building block}, thus the injected malware resembles a set of malware basic blocks, whose execution is controlled either by a static configuration file or by a remote server. In either case, the malware communicates with a remote server to transfer back data and/or results of completed actions.

Intensity of malicious behavior is controlled on two levels: network level and local level (intensity of a malware basic block). Network level has two parameters: the size of data chunk being transmitted and the delay between two consequtive transmissions. On the local level, the number of parameters controlling intensity varies, and it depends on a malware basic block. In other words, each malware basic block has its own set of parameters. Usually, the program code that carries out a particular malicious action is divided into a few parts and a delay is inserted between these chunks of the code. Thus, many malware blocks have a {\it delay} parameter in their configuration file. For example, the malware basic block that carries out DDoS attack has a few local intensity paramters: delay between requests, amount of data sent in each request, it also has a set of ip addresses of the hosts under attack as well as the number of requests or the longitude of the attack.

Malware basic blocks and the summary of their specific parameters are presented in the table ~\ref{mal_gen}. Stealing text messages comes in two flavors: it could be done online or offline. The online version implies analysis of incoming messages, forwarding some of them to the attacker and removing them from the device. This method is used by real malware to intercept authentication messages coming from financial institutions. The offline method of stealing text messages means uploading all or some of the currently present on the device messages to the attacker's server. When stealing browser data, the synthetic malware can transmit to the attacker's server browser history and/or bookmarks. Such information can be used by an attacker to learn user's interests and preferences. Also, our malicious payload can steal the entire files or the content of particular folders (SD card subcategory). Emulation of a real malware that turns a device into a net node is achieved through the following two activities: downloading files and DDoSing network hosts. Computationally intensive workload is represented by multiplication of two random matrices, whose parameters are defined in the configuration file.

Based on the comprehensive analysis of the existing Android malware and of the underlying black market economy, we chose the most widespread malware types that are prevalent today and very unlikely to become extinct in the near future. The goal of our research is not only to develop a lightweight detection system, but also to study how malware may adapt to such detection schemas. The only way for a malware to escape detection is to hide itself within a benign activity. In order to study such effect we built a malware generator with numerous parameters controlling the intensity of the malicious behavior.

\ignore{
\begin{table}[ht] 
\caption{Highlevel classification} % title of Table 
\centering % used for centering table 
\begin{tabular}{c c c c} % centered columns (4 columns) 
\hline\hline %inserts double horizontal lines 
Year & Info. Stealers & Net Nodes & Comput. Nodes \\ [0.5ex] % inserts table 
%heading 
\hline % inserts single horizontal line 
2013 & 38\% & 32\% & 0 \\ % inserting body of the table 
2012 & 57\% & 60\% & 0 \\ [1ex] % [1ex] adds vertical space 
\hline %inserts single line 
\end{tabular} 
\label{table:highlevel_classification} % is used to refer this table in the text 
\end{table} 


\begin{table}[ht] 
\caption{Info Stealing} % title of Table 
\centering % used for centering table 
\begin{tabular}{c c c} % centered columns (4 columns) 
\hline\hline %inserts double horizontal lines 
%Subcategory & \multicolumn{2}{c} Info. Stealers & \multicolumn{2}{c}Net Nodes \\ [0.5ex] % inserts table 
%heading 
subcategory & 2013 & 2012 \\
\hline % inserts single horizontal line 
 phone info & 65\% & 66\% \\ % inserting body of the table 
 sms        & 58\% & 46\% \\ % inserting body of the table 
 contacts   & 53\% & 33\% \\ % inserting body of the table 
 apps info  & 30\% & 13\% \\ % inserting body of the table 
 GPS        & 27\% & 18\% \\ % inserting body of the table 
 email      & 19\% & 8\% \\ % inserting body of the table 
 browser    & 19\% & 10\% \\ % inserting body of the table 
 files      & 15\% & 13\% \\ [1ex] % [1ex] adds vertical space 
\hline %inserts single line 
\end{tabular} 
\label{table:info_stealers} % is used to refer this table in the text 
\end{table} 


\begin{table}[ht] 
\caption{Net Node} % title of Table 
\centering % used for centering table 
\begin{tabular}{c c c} % centered columns (4 columns) 
\hline\hline %inserts double horizontal lines 
%Subcategory & \multicolumn{2}{c} Info. Stealers & \multicolumn{2}{c}Net Nodes \\ [0.5ex] % inserts table 
%heading 
subcategory & 2013 & 2012 \\
\hline % inserts single horizontal line 
 down. files & 50\% & 83\% \\ % inserting body of the table 
 scam 	     & 35\% & 6\% \\ 
 DDoS        & 10\% & 6\% \\ % inserting body of the table 
 add clicker & 5\%  & 0\% \\ [1ex] % [1ex] adds vertical space 
\hline %inserts single line 
\end{tabular} 
\label{table:net_node} % is used to refer this table in the text 
\end{table} 


\begin{table}[ht] 
\caption{Synthetic malware generator} % title of Table 
\centering % used for centering table 
\begin{tabular}{c c c} % centered columns (4 columns) 
\hline\hline %inserts double horizontal lines 
%Subcategory & \multicolumn{2}{c} Info. Stealers & \multicolumn{2}{c}Net Nodes \\ [0.5ex] % inserts table 
%heading 
malware basic blocks & ~ & ~ \\
\hline % inserts single horizontal line 
Info stealers & ~ & ~ \\ 
\hline % inserts single horizontal line 
 sms 		& online & offline \\ % inserting body of the table 
 phone info 	& ~ & ~ \\ 
 contacts       & ~ & ~ \\ % inserting body of the table 
 GPS 		& ~ & ~ \\
 browser info 	& history & bookmarks \\ 
 SD card 	& files & dir content \\ 
 apps info 	& ~ & ~ \\ 
\hline % inserts single horizontal line 
Net node & ~ & ~ \\ 
\hline % inserts single horizontal line
 download 	& file(s) & ~ \\ 
 DDoS 		& IPs & ~ \\ 
\hline % inserts single horizontal line 
Comput. node & ~ & ~ \\ 
\hline %inserts single line [1ex] % [1ex] adds vertical space 
matrix mult 	& A & B \\ [1ex] % [1ex] adds vertical space 
\hline %inserts single line 

\end{tabular} 
\label{table:mal_gen} % is used to refer this table in the text 
\end{table} 

}


==> real-malware.tex <==
\section{Reverse Engineering Real Malware}
\label{sec:rev-engg}

In this section, we present experiments with real malware samples and discuss
issues with running them in a controlled environment. Our results demonstrate
that our approach is more effective for detecting real malware rather than for
synthetic samples. This is because real malware developers  do not try to hide 
malicious behavior. Similar to our malware classification, we use at least one
sample to represent each category. 

\subsection{Infostealers}

For our experiments we chose Trojan-Spy.AndroidOS.Geinimi.a (MD5
e0106a0f1e687834ad3c91e599ace1be) and Backdoor.AndroidOS.Sinpon.a (MD5
d4a557ec086e52c443bde1b8ace51739). None of these samples unmodified. Typically,
malware checks the runtime environment used to execute Android apps (ex.
geographic location and other IDs). The goal of these checks is to detect
whether a malware is executed within an emulator or in a geographic region
where it is not supposed to work -- implying that someone is trying to reverse 
engineer the malware-ridden application. If something suspicious is detected,
the malicious payload is not executed and the underlying application operates 
normally. It is important to note that the main difference between a repacked,
malicious applicatoin and the corresponding original application is the
malicious component.

We found a Geinimi.a sample embedded within a repackaged version of the computationally
intensive game MonkeyJump2. Geinimi.a is a complex and heavily obfuscated malware family. 
Besides emplying obfuscation it also encrypts almost all strings
and uses Java reflection for dynamic method invocation. These are all features
impede reverse-engineering Geinimi.a.  The Geinimi.a malware mainly focuses on
stealing personal information, but also posseses the capability to install 3rd
party apps. Thus, it is able to execute other attacks. 

Analysis of the network traffic generated by the sample showed that its
supporting C\&C is no longer functioning. The Geinimi.a sample tried to connect
to the C\&C server every 5 min to check whether or not to issue any commands on 
the host system. Since we did not observe any replies from C\&C server, we wrote 
our own C\&C server and added instrumentation code to make sure that malicious 
payload is actually issued. All communication with Geinimi.a malware is encrypted 
using 52-DES with a hardcoded key 0x0102030405060708. 

The interesting feature of Geinimi.a is that it split all incoming commands in one 
of the two groups. From semantic point of view, they are almost identical, but their 
internal implementation is different. It is worth noting that some of them are not 
completely implemented. We exercised 9 commands of one type; for 8 of these commands 
the difference in their implementation is negligible and thus insignificant for our 
experiments. The last command, downloading and installation of an app, is implemented
differently across these two groups, but only one version works reliably.

We had to modify portions of Geinimi.a sample due to lack of necessary hardware and
bugs within the Ginimi.a code. When first running the app infected by Geinimi.a, 
when the malware woudl try to access the cellular network location service it
would crash. The lack of this hardware component on the Arndale board and no
hardware stub to spoof it caused the program to crash. We replaced access to network 
service with access to the GPS service. 


The original code was able to extract all of the text messages, encrypted them,
and write to an open Java socket, but not commit them. To fix this partial execution,
we augmented the to guarrantee the text message committing. When testing the 3rd party 
program installation functionality, we observed that the malware failed silently 
because it could not write to SD card (Android boots off the SDCard on the
Arndale board and an extra partition on the card was not made to spoof it). We
modified the code to store downloaded APK files in the /data folder  and 
automatically set the required permissions instead. 
version.

The other infostealer we studied represents the Sinpon.a malware family. 
It is capable of executing 20 different commands from a C\&C server and can send
sensitive data back to the C\&C server. As in the previous case, C\&C server did
not appear to be alive so we implemented our own C\&C server that supported 
Sinpon.a’s protocol. 

We found out that Sinpon.a did not run on Android 3.0 and above because since
Android 3.0 Google has prohibited establishing network connection within the
app’s main thread. Thus, we had to modify the byte code in order to execute
Sinpon.a on Android 4.2.1. We embedded Sinpon.a in three apps: Angry Birds,
Sana med. app and TuneInRadio.

\subsection{Click Fraud} 

In this experiment we used the sample that is identified as
AdWare.AndroidOS.FetGp.a (MD5 5b5f65e1d014dbb8e55602ed468cb5eb) by Kaspersky 
rRantivirus.The malware pretends to be a Google Play app, but
it does not do anything useful. When a user launches the app, it shows only a
white screen, and at the same time it starts a background service that keeps
running even after the app is closed. The background service registers the mobile
device by contacting http://www.mobilefilmizle.com/ipzaman.php and this server
is checks the devices’s network configuration and if the device’s IP address has changed. 
The service then sets a timer to wakeup event every 2 minutes. When the
application awakes, it contacts the other server to retrieve a set of keywords which 
are later entered into Google one-by-one. The malware opens the search results
for each query and scrapes the result page for links containing a certain format
to click them using JavaScript mouse events. This allows the malware clicks on a 
lot of advertising links, generating money for its developers When testing the 
sample, we made sure that its C\&C server was alive by capturing network traffic and 
instrumenting Dalvik bytecode to spoof the command on subsequent calls. We embedded 
Sinpon.a in three apps: Angry Birds, Sana med. app and TuneInRadio.

\subsection{Computational Workload}

We have not observed computationally intensive malware in the wild, that’s why
we obtained a real MD5 descriptor (password cracker) from Google Play (MD5
b7f53ff767e130758a6375315e62e82a). The app uses brute-force search to break the
MD5 hash of a password. We injected the code into legal version of AngryBirds,
Sana, and TuneInRadio.



==> related.tex <==
\subsection{Offline Static and Dynamic Analyses}
\label{sec:offline}

Mobile platform providers like Google and Apple 
%require developers to register
%using a key-pair and check whether application binaries are signed by
%registered developers when installing applications (`apps') on phones. While
%registration acts as a mild deterrent to attackers,
%Apps are then isolated from each other on users' phones.  such as checking
%developer-signatures on binaries registered in the app-store and  per-app
%isolation on the device. Beyond these measures, both commercial and academic
%defenses against mobile malware include Before publishing an app to the
%app-store, 
use static and dynamic program analyses to analyze an app's
code and program executions respectively before publishing the app to their
app-stores. 

	



The simplest static analyses look at each app's permissions to access sensitive devices in order
to detect
overprivileged apps~\cite{android-demystified}. Others detect malware repackaged in
benign apps through pairwise comparison of
binaries~\cite{DNADroid,DroidMOSS,Juxtapp,PiggyApp}, or use
type-systems~\cite{ernst-taint-type} and program dependency
graphs~\cite{apposcopy} to detect malware.  
%However, simple permissions-analyses are inconclusive
%since even simple applications need access to sensitive permissions like
%internet access, location (to support advertisements), and even to SMSs (to
%automate two-factor authentication). 

However, static analyses are commonly evaded by malware that encrypts all
static strings in the code~\cite{malware-str-enc}, uses Java reflection to
obfuscate program execution~\cite{malware-obfuscate-xuxian}, or leaks
secrets through the underlying system and hardware through timing and covert
channels~\cite{android-covert-channels}. Further, static analyses cannot
analyze apps that load code dynamically, e.g., as Java classes or through
web-views~\cite{webview-attacks}.

Dynamic analyses
observe an app's run-time data to  
 enforce access control or information flow policies~\cite{DroidScope,XuSA2012,HornyackHJSW2011,taintdroid}.
Droidscope~\cite{DroidScope}, for example, reconstructs OS-level and Java-level semantics of
Android apps and enables developers to specify rules for malicious/benign
behaviors.  Dynamic information flow tracking mechanisms~\cite{taintdroid}
%enforce  security policies within Android apps at runtime, e.g.,
label sensitive data (such as Contacts) and alert users when sensitive data is
sent outside the device.
%should never be read by a wallpaper app.  
Aurasium~\cite{XuSA2012} repackages existing apps by attaching user-level
sandboxing and policy-enforcement code.  
%AppFence~\cite{HornyackHJSW2011} An alternative approach is to substitute
%shadow data for user-sensitive data.  and blocks network transmissions that
%contain on-device use only data.  While these dynamic analyses provide
%mechanisms, {\em policies} for labeling sensitive data and enforcing
%information flows are left to the users/analyst.  Further,

Unfortunately, dynamic approaches too can be evaded using conditional execution
(`implicit flows') to leak sensitive data~\cite{tainting-pointless}. They also
slow down apps as the security checks execute at run-time. Hence,
dynamic analyses are used offline by driving apps on emulators using artificial
inputs~\cite{dynodroid,concolic-android,droidfuzzer,guided-gui-testing}.
%Since these analyses are slow, they are used offline and 
Such offline analyses cannot detect malware
exploits that succeed in the field due to user- or developer-errors.





\ignore{
{\bf Android Security.}
Zhou et al.~\cite{dissect_malware_2012}
presents a comprehensive survey of Android malware. The authors analyze and classify more than
1,200 Android malware samples using a variety of criteria, and estimate that 86\% out of 1,200
samples they analyzed were repackaged. The straightforward approach for
detecting repackaged malware is to develop an algorithm that can do pairwise
comparison of apps to find the original app. DNADroid~\cite{DNADroid} extracts a program
dependency graph (PDG) from Android apps and compares them in terms of PDGs.
DroidMOSS~\cite{DroidMOSS} applies fuzzy hashing to app comparison problem. 
Juxtapp~\cite{Juxtapp} uses k-grams of opcode sequences of Android apps and feature-hashing
approach. One disadvantage of such algorithms is the lack of
scalability. PiggyApp~\cite{PiggyApp}
proposes a decoupling technique to separate primary and piggybacked modules,
feature fingerprint to extract semantic features, and a linear arithmetic search
algorithm to deal with scalability issues.

\ignore{Another set of security tools analyzes the semantics of Android apps though
their dynamic behavior. Droidscope~\cite{DroidScope} reconstructs OS-level and Java-level
semantics of Android apps and is a platform for developing high-level
tools for security purposes.} Tools exist that enforce security policies
within Android apps at runtime, e.g., TaintDroid~\cite{taintdroid}. 
Aurasium~\cite{XuSA2012} repackages
existing apps by attaching user-level sandboxing and policy-enforcement code.
AppFence~\cite{HornyackHJSW2011} substitutes shadow data for user-sensitive data and blocks network transmissions that contain on-device use only data. 

%Several solutions rely solely on static methods of code protection (e.g., obfuscation).
%such as obfuscation and/or encryption. 
%The most widespread way to protect Android
%apps is to use Google’s ProGuard ~\cite{GoogleProGuard}, which is a part of Android SDK. There is
%another commercial obfuscator called Shield4j~\cite{Shield4j}. Google puts efforts into promotion of application licensing ~\cite{GoogleAppLicensing}, but it has
%been demonstrated to be broken.

\ignore{Triceratops~\cite{Triceratops} proposes hardening of Android apps via
splitting an app into verified and unverified regions through conservative
static analysis. Then it patches the unverified region with code based on the
supplied security policy. The inserted code is used for dynamic checks whether
the app complies with the imposed security policy. AppInk~\cite{AppInk} utilizes dynamic
graph-based watermarking that inserts transparent watermarking into an app and
generates a manifest app that can recognize watermarks and detect code
modification. Stowaway ~\cite{android-demystified} tool maps API calls
to requested permission and thus detects overprivileged apps.
}

}

%{\bf Hardware computational signals.} 
%The most relevant paper to our project is 

This paper builds on the seminal work by Demme et
al.~\cite{perf_counters_2013}, which proposes the use of hardware performance
counters for online malware detection. The authors key insight is to train a
classifier for known malware and arbitrary benign apps and shows a true
positive rate of 80\% for a false positive rate of 20\% (excluding {\tt netd}).
We discuss the differences in our evaluation methodology in the
Sections~\ref{sec:intro} and \ref{sec:pitfalls}, and it is fallacious to
superficially compare our raw true positive and false positive rates (they are
similar) since our datasets are very different.  We also evaluate \name using
anomaly detectors instead of signatures.

% algorithms
%detect anomalies (not sig
%we focus on
%identifying the break-even point for each algorithm

%However, our datasets are very differe

 
%Their malware-signature
%detection technique is best suited to detect {\em known} malware samples and
%complements our anomaly-based approach that models benign apps.  Our evaluation
%methodology is significantly different -- instead of executing off-the-shelf
%malware samples, we stress test our anomaly detector using a) a diverse set of
%extant and synthetic malware whose payload is confirmed to execute correctly so
%that we can know {\em which} payloads are detectable, and b) comparing
%repackaged malware executions with those of their baseline app  to evaluate
%false positives.  

Hardware based anomaly detectors have been proposed in
concurrent work by Tang et
al.~\cite{anomaly-detector-columbia-raid} targeting desktop malware.  
Our evaluation methodology is significantly broader (beyond qualitative 
differences in mobile payloads v. desktop exploits 
as discussed in Section~\ref{sec:mobile-uniq}). 
We evaluate our algorithm using 66
mobile malware payloads in 9 mobile applications with 1--2 hour traces while
they use 3 exploits and Stage 1 and 2 payloads embedded in 2 benign
applications. While they conclude adapting exploits is extremely hard
for an attacker, we construct an adaptive malware payload suite.
Our anomaly detection algorithms (feature selection and model building)
is also different -- overall, we believe their approach towards detecting
malware exploits due to common exploit-kits is complementary to our
payload based mobile malware detection.

%As such, our work on {\em mobile} malware has significant
%differences 
%(Section~\ref{sec:mobile-uniq})  

%Tang et al.  propose a very different algorithm for extracting
%features and building the model, and evaluate their detectors using {\em
%desktop malware} generated using the metasploit tool.  Instead, our pipeline
%uses DWT to extract features from coarse-grained phase information  and Markov
%or bag-of-words based models.  

%On the other hand, we fix the 6 performance counter signals (since
%realistic experiments on a board take time) while they do a careful sweep of
%performance counters to find best ones. 
%-- which execute regular code but out of context -- whereas their goal
%s to detect abnormal code typical of {\em exploits}.

%Power traces are another complementary hardware level
%signal~\cite{energy-anomalies, virus_meter, clark-healthtech13} to analyze
%energy consumption of mobile devices and medical software and try to detect
%malicious activity.
%
\todo{v. Tang -- metasploit with one well known shell code -- payloads are
diverse and can look like apps. Quantify this! Web browser only as the
baseline.}

%, we test a diverse set of popular apps under realistic usage
%for over 1 hour each. 

%hey evaluate their
%framework at much coarser granularities - thread- and package-level detection -
%by averaging the classification probabilities of all data points. In
%comparison, HaCS is designed to provide almost real-time detection and it works
%at the granularities of 50-150 ms (Markov model) and 1500 ms (BoW).  Also, we
%overcome the problem of separating malicious threads from benign ones within an
%app by operating at the process level. 
%
%Second, we demonstrate how to model different apps' behavioral 
%aspects (statistical and temporal) simulteniously (sec. 6.6) instead of using machine learning 
%algorithms as a black box. Third, our detection rate is higher at the fixed level of false positives~\ref{fig:boosting-table} 
%than the thread-level accuracy in (Fig. 4 Excluding 'netd')~\cite{perf_counters_2013} (we compare 
%with thread-level detection because it is the most fine grained level presented in ~\cite{perf_counters_2013}).
%And finally we try to understand what makes Android malware to stand out on the microarchitectural level and 
%the limits of the computational signatures by constructing an adaptive malware.
%}
%

\ignore{
The authors postulate the possibility of using
performance counters to detect known Android malware using malware-signatures.
This technique is best suited to detect {\em known} malware samples and
complements our anomaly-based approach that models benign apps.  Our evaluation
methodology has a very different focus. Instead of executing off-the-shelf
malware samples, we stress test our anomaly detector using a) a diverse set of
extant and synthetic malware whose payload is confirmed to execute correctly,
and b) comparing repackaged malware executions with those of their baseline
app.  To evaluate false positives, we test a diverse set of popular apps under
realistic usage for over 1 hour each. 
}
%Identifying which combinations of payloads and benign apps
%do {\em not} work well 


%
%accuracy of malware detection carried out by classifiers.
%
%Clark ~\cite{clark-healthtech13} analyze energy consumption
%of medical software and found that even such a coarse-grained method can detect
%malware infecting an embedded WinXP system. 
%
%Although we incorporate previous ideas -- machine learning for dynamic
%analysis and the use of performance counters as a signal -- 
%Our approach is complementary to the above prior work.


\ignore{
========

Citations/links to be added for intro and background:

- Web-view vulnerabilities - Erica Chin paper

- Ad-vulna - Fireeye blog

- Google verify -  http://qz.com/131436/contrary-to-what-youve-heard-android-is-almost-impenetrable-to-malware/

- Breaking Google bouncer: https://www.duosecurity.com/blog/dissecting-androids-bouncer

- 50B app downloads and 1B mobile device activations.
http://www.theverge.com/2013/7/24/4553010/google-50-billion-android-app-downloads-1m-apps-available

- discontinued apps as malware:
http://blog.trendmicro.com/trendlabs-security-intelligence/trojanized-flappy-bird-comes-on-the-heels-of-takedown-by-app-creator/
}
\ignore{
All virtualized phone instances in the Bouncer are associated with the same account and have exactly one contact and two photos on the simulated device.
Bouncer only checks a submitted app for five minutes.
Bouncer only does dynamic analysis. This means only applications misbehave when running in the Bouncer will get caught.
Google’s IP range assigned to Bouncer can be revealed as the analyzed apps are allowed to access Internet while being tested.

Update attack: No malicious code needs to be included in the initial installer.
In this case, the app can have an even better chance to evade Bouncer’s
detection. Once the application passes Bouncer’s check and gets installed on a
real user’s device, then the application can either download additional
malicious code to run or connect to its remote control and command (C\&C) server
to upload stolen data or receive further commands. Just this month, another two
fake apps successfully avoided Bouncer using this technique and snuck into Google
Play, staying there for two weeks. (We detect these apps as
ANDROIDOS\_TROJDOWNLOADER.A and ANDROIDOS\_TROJSMS.A.)

http://blog.trendmicro.com/trendlabs-security-intelligence/a-look-at-google-bouncer/

http://blog.trendmicro.com/trendlabs-security-intelligence/infographic-behind-the-android-menace-malicious-apps/

Classification: 
Adware pushes ads as urgent notifications.
Spying tool sends out GPS location and tracks text messages and call logs.
Rooter allows attackers to send commands to compromised devices.
Data stealer steals and sends different information to the command and control server.
Premium service abuser subscribes infected phones to premium services without consent.
Click fraudster abuses mobile devices via pay-per-click online ads.
Downloader downloads other malware or benign applications onto infected devices.

As we noted earlier, the number of mobile malware threats has crossed the 1
million mark, and as of the end of 2013 stood at almost 1.4 million malicious
and high-risk apps. We believe that by the end of 2014, this number will be at
over 3 million.  The proportion of mobile malware with some sort of
information-stealing ability grew from 17\% at the start of 2013 to almost a
quarter by year’s end.  Overall, about a fifth of all mobile malware had some
sort of information theft capability.

http://blog.trendmicro.com/trendlabs-security-intelligence/looking-forward-into-2014-what-2013s-mobile-threats-mean-moving-forward/

50B app downloads and 1B mobile device activations.
http://www.theverge.com/2013/7/24/4553010/google-50-billion-android-app-downloads-1m-apps-available

Verify Apps intervenes when an app is downloaded, compares it to a large
database of malware information curated by Google, and warns the user if the app
is potentially harmful.  Using Verify Apps, Google collected app installation
data outside of the protected perimeter of the Google Play app store from
installations “in the wild,” where the incidence of malware is higher. Only
0.12\% of users chose to ignore the warnings and install potentially hazardous
apps, i.e., 1.8M malware installations from 1.5B downloads outside the official
Google store. These were 40\% fraudware, 40\% rootware, and 15\% spyware.
http://qz.com/131436/contrary-to-what-youve-heard-android-is-almost-impenetrable-to-malware/

% In 2012, 17 malicious apps were installed 700k times before their removal.

Even a few malicious apps can be installed over 100k times before their removal~\cite{trendmicro-12}. 


====




The feasibility of online malware detection using only performance counters has been discussed in ~\cite{perf_counters_2013}. The authors implemented a blacklist approach: they trained a set of classifiers on samples belonging to a particular malware family (each family had a few classifiers). Later, they tested their approach on previously unseen malicious samples. First, their approach has similar limitations to the limitations of static signature scanners: someone has to analyze malware samples and partition them out into different families, then those samples can be used for training a classifier. A few dozen malware families exist, and this means that current readings from PMU should be processed simultaneously by a few dozen classifiers; however, this makes the approach inapplicable to the deployment on real devices because the classifiers would consume lots of energy and computational resources. Second, the authors of ~\cite{perf_counters_2013} did not ensure that malware actually executed in their experimental environment. Usually, every malware sample contains multiple functions that check the properties of the runtime environment, and quite often those checks fail. If they fail, the microarchitectural footprint of a crashed malware is significantly different from a normal application. This might mean that the results published in ~\cite{perf_counters_2013} are biased.

SimPoint ~\cite{bblock-phases}, ~\cite{auto-prog-behavior}, ~\cite{wavelet-phases} is the other project whose results we reused in the current work. SimPoint introduced the notion of execution phases and demonstrated their applicability to simulation problems. The authors explored automatic approaches to analysis of phase behavior within compilable programs. Conventional programs go through a sequence of phases during their execution, and such phases can be detected using binary code analysis or microarchitectural events. In the original project, the detected phases were used to speed up hardware simulations. We significantly extended the previous work by applying phase detection to managed languages and applications that are involved in complex interactions with OS level components.

There are a few other projects that were insightful, but not directly related to our research. In those projects, researchers analyzed the possibility of malware detection using a power channel. We think that the power channel provides less information than performance counters (at least, it is hard to ascribe power consumption to a particular process ~\cite{power_patterns}). In all cases, the authors did not consider full-fledged systems (e.g., medical devices or very aggressive types of malware executed on old platforms). ~\cite{clark-healthtech13} explored the possibility of using simple statistical metrics to detect malware running on medical devices. Such an idea would not work in our case because of the large variety of concurrently running processes. ~\cite{energy-anomalies} and ~\cite{virus_meter} demonstrated good detection results on few very energy-greedy malware samples or plain samples executed in the system with low background noise.

}




==> results2.tex <==
\begin{figure*}[t]
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/12.signature/AngryBirds_RANDOM_FOREST_ROC.pdf}
\label{fig:sign-roc}
  \end{minipage}
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/12.signature/AngryBirds_RANDOM_FOREST_auc.pdf}
\label{fig:sign-auc}
  \end{minipage}  
  \caption{ Training should be accomplished on a balanced data set. Across all the apps in our corpus the average difference between "Same Malware" AUC vs "Other Malware" AUC is 15\%.}  
\label{fig:GD_ROC}
\end{figure*}

\begin{figure*}[t]
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/13.power_transform/AB_original_counter_7.pdf}
\label{fig:sign-roc}
  \end{minipage}
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/13.power_transform/AB_power_transformed_counter_7.pdf}
\label{fig:sign-auc}
  \end{minipage}  
  \caption{ Distribution of load/store events before and after power transform with $\lambda=0.28$. In comparison to exploits, power transform does not make malicious payloads more discernible from benign behavior.
.}  
\label{fig:GD_ROC}
\end{figure*}

%%%%%%%%%%%%%

We first show that both benign apps as well as the malware payloads have
diverse hardware signals. This quantifies the design choices made in
Sections~\ref{sec:malware-gen} and~\ref{sec:apps-inputs} 
and establishes that our 
detection results are not skewed in favor of or against the HMD. 
%Ensuring that the population of the \name is diverse
%
%Establishing that the population of programs in the \name is diverse is
%important


We then present the detection result matrices and false positive rates for both
the Markov-based and the bag-of-words based HMDs. We plot increasingly distinct
malware payloads v. each benign app as a heatmap, and identify the detection
threshold for each pair of malware and benign apps. We further show that both
HMD classifiers can detect malware within a few seconds of the start of
malicious behavior, and can be stored on a mobile device in only a few KBs of
memory.
%

\todo{False positives?}

Finally, 
%we also demonstrate that the dynamic analysis of HMDs complements static
%analyses employed by platforms like Google today. In particular,
we show that techniques such as (Java) reflection that are employed by malware
to throw off static program analysis~\cite{Livshits_Reflection_Java} in turn make the malwares'
(dynamic) hardware signals {\em more} distinct. 
%This is an interesting result and shows that HMDs can complement 
HMDs thus complement static analyses deployed in the field today.


%\vspace{-0.1in}
\subsection{Diversity of Baseline Apps}
\label{ben-app-diversity}

%We first investigated whether the nine baseline applications that we had chosen
%are sufficiently diverse. To quantitatively analyze the diversity of the apps,
%We can see that the benign apps in \name 

We use principal component analysis (PCA) to
%visualize the distribution of 
project the benign hardware signals 
into a 2-D space (Figure~\ref{fig:baseline-diff}). 
The top two dimensions here 
retain 90.77\% of variability in the data. The apps are distributed 
evenly
over the region and do not form clusters -- this indicates that 
the 9 benign programs we have chosen have diverse hardware signals.
%as underlying benign apps are diverse with respect to
%their low-level characteristics.


To further confirm the diversity in their hardware signals, we compare the
benign apps using the Markov model based anomaly detector -- if the apps are
diverse, we expect that a model trained on one app's hardware signals will
label the others' signals as an anomaly.
We illustrate this comparison using three apps -- AngryBirds, Sana, and
TuneInRadio -- that represent computationally
intensive, user-driven, and network intensive apps respectively.

Figure~\ref{fig:baseline-diff} shows true positives v. false positives rates 
computed using 80ms program phases. The steep step-like curves indicate that
new apps are accurately identified as anomalous: a 80--100\% true positive
rate for a 10--20\% false positive rate.
%(i.e., each phase is mapped to a
%state from sec.~\ref{sub:representation}).  
We also see that the dissimilarity measured this way is
not symmetric, which follows from the probabilistic nature of the Markov
models and the noise in the input data. 
%

Interestingly, this experiment also shows that it is easier to distnguish
hardware signals from completely different apps -- as in prior
work~\cite{simha-isca,map} -- in comparison to
separating out a parent app's traces with and without malicious phases
interleaved within them. 

Finally, we note that the malicious payloads too have diverse hardware signals.
In addition to the behavioral diversity described in
Figure~\ref{fig:synthetic-malware}, we projected their hardware signals using
PCA in two dimensions (graph not shown to save space) and ensured that the
signals were spread out without forming clusters. 


%%%%%%%%%%%%%
%\vspace{-0.1in}
\subsection{Results for Markov Model HMD} \label{sec:markov-results}

%-----------------
\begin{figure}[tbp]
%\vspace{-0.2in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/6.heat_map/MM_heat_map.pdf}\par
\caption{Determining the operating range of Markov model HMD. 
In each rectangle, the size of malicious payload grows from
the top to the bottom, and the amount of delay decreases
from left to right (H=High, M=Medium, Z=Zero delay). If color goes from light to dark within a rectangle,
then the detection threshold (i.e., the lower end of the operating range) lies inside the rectangle. 
%Apps with repeating behaviors like TuneIn Radio
%yield best results. Compute-intensive dynamic apps like CNN hide malware better.
}
\label{fig:synthetic-MM-heat-map}
\end{figure}
%-------------------

Figure~\ref{fig:synthetic-MM-heat-map} shows the results-matrix for the Markov
model based detector. Each cell in the matrix corresponds to a malware payload
action (y-axis) and benign app (x-axis) pair. The malware payloads are grouped by
category and within each category, increase in size from top to bottom
and in delay from right to left.  
%We use three levels of delay: zero, medium and high (they are denoted by the
%symbols "N", "M" and "H" at the bottom of the heat map). The small white cells
%with an "X" indicate that we did not conduct that experiment.  That is, we
%tested the ID+GPS stealer using only two type of delays -- zero and medium --
%because even zero delay makes detection really hard due to negligible
%computational overhead. The parameters on payload size 
These experiments use parameters from 
Figure~\ref{fig:baseline-apps}.
The intensity of the color -- from light green to dark red --
corresponds to the detection rate, which is computed as the number of raised
alarms versus the total number of alarms that could be raised. All the
results are shown for a false positive rate of 20-25\%.
%-----------------
\begin{figure}[tbp]
%\vspace{-0.2in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/6.heat_map/SVM_heat_map.pdf}\par
\caption{
Determining the operating range of Bag-of-words HMD.  
Interestingly, the bag-of-words model performs better than
Markov model for compute intensive and dynamic apps (e.g., Angry Birds, CNN, and Zombie
WorldWar). }
\label{fig:synthetic-SVM-heat-map}
\end{figure}
%-------------------

%For most pairs of malware categories and benign app,
\noindent{\bf Operating range (Figure~\ref{fig:synthetic-MM-heat-map}).}
Increasing the size of each payload action makes malware more detectable --
this can be seen as the colors being more intense towards the bottom part of
most rectangles.  Increasing the delay between two malicious actions does not
have a similarly predictable effect -- SMS stealers in Angry Birds is a rare
pair where detection rate increases with delay. This is interesting since
intuitively, adding delays between payload actions should decrease the chances
of being detected. However, these experiments indicate that for most
malware-benign pairs, detection depends on how each payload action interferes
with benign computation rather than delays between the payload actions.  The
most important take-away from Figure~\ref{fig:synthetic-MM-heat-map} is that for
most malware-benignware pairs, the detectability changes from light green to
dark red as we go from top to bottom in the rectangle -- this shows that our
malware parameters in Figure~\ref{fig:synthetic-MM-heat-map} are close to the 
detection threshold, i.e. the lower end of the HMD's operating range for the
current false positive rate. 
There are a few exceptions as well, such as
click fraud, DDoS, and password crackers hiding in CNN; and
DDoS in Angry Birds, Maps, Translate, and Zombie World Wards. For these cases,
the payload intensity has to be increased further to find their 
detection threshold.


\ignore{%red}{REMOVE THIS
	%-------------------
	\begin{figure}[tbp]
	\vspace{-0.2in}
	   \centering
	   \includegraphics[width=0.45\textwidth]{figs/apk-30-sec.eps}\par
	\caption{(Markov model) Malware-level true positive versus 30-sec false positives: detection accuracy for synthetic malware.}
	\label{fig:synthetic-malware-phase}
	\end{figure}
	%-------------------

	\noindent{\bf False positives (Figure~\ref{fig:synthetic-malware-phase}).}
	%To evaluate overall performance of the detector, we generated traditional ROC
	%curves (Figure~\ref{fig:synthetic-malware-phase}).
	%Figure~\ref{fig:synthetic-malware-phase} 
	We measure the percentage of detected malware samples (TP rate) versus the
	number of false alarms (FP rate) raised on per 30-sec window basis. 
	%The 30-sec time window represents one (arbitrary) session of using an app
	If an alarm is raised within a 30-sec window, the entire window is considered
	to be malicious by our malware detection scheme. We chose 30-sec as the
	duration since apps do not come with a pre-defined or shared ``session'' of
	expected usage. For usage traces longer than 1--2 hours per malware-benign pair,
	results can be showed in larger time units.
	%
	Overall, we find that our Markov model HMD works best for apps with predictable
	(i.e., simple or regular) behavior. The top three curves, corresponding to the
	Amazon, Firefox and TuneInRadio apps, have ~17\% FP for ~88\% TP. 
	%
	While CNN seems conceptually similar to Amazon, 
	%we do not achieve as good detection for CNN as for Amazon.  This may be
	%because 
	its CNN's dynamic behavior is more variable.  In addition to text news and
	static ads, CNN shows pictures and plays videos, animated ads etc.  CNN and the
	game Zombie WorldWar show
	%in terms of the scalability of the 
	worst TP v. FP results, i.e.  allowing for more false positives improves their
	malware detectability insignificantly.  Hence these apps are much more
	attractive to malware developers to use as a parent app.
	%
	Detection rates of the remaining apps cluster around Sana's curve. One may
	expect that Sana's simple interface makes detection easy.  However, its
	user-driven nature creates short and sharp spikes within the traces, which
	could not be reliably captured by the Markov model. For most applications, the
	Markov model can reliably detect from 30\% to 90\% of malware samples while not
	exceeding a 10\% false positive rate.
}

%-------------------
\begin{figure}[tbp]
%\vspace{-0.1in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/5.ttd/signatures.png}\par
\caption{(Markov model) Time to detection and signature sizes for each baseline app.}
\label{fig:time-to-detect}
\end{figure}
%-------------------

\vspace{0.2in}
\noindent{\bf Detection Time and Space Overheads
(Figure~\ref{fig:time-to-detect})}
%We provide insights into what overhead could a detector based on Markov model
%We quantify the cost of a Markov model HMD on hardware, network 
%For this purpose we computed 
Markov models representing the behavior of the benign apps
(Figure~\ref{fig:time-to-detect})  vary from 1.2KB to 6.7 KB, with an average
size of 3.2KB -- they are thus cheap to store on devices and transfer over
cellular networks. 

%Such small sizes make storing and
%transferring signatures. and their enforcement at runtime is
%unlikely to cause significant overhead.

The time to detection parameter for an HMD characterizes how quickly it can
react to an ongoing attack.  We measured this parameter by starting our malware
detector and malware sample simultaneously.  Time to detect parameter depends
on the number of states in the Markov model, the length of \textit{phase\_windows} and
the number of subsequent states to be observed before the detector optionally
raises an alarm.

Figure~\ref{fig:time-to-detect} shows that time to detection ranges between 1.2
seconds to 4.4 seconds and about 2.5 seconds on average.  This means that the
system can detect suspicious activities at the very beginning, considering
that exfiltrating even one photo takes 2.86 sec on average.


\subsection{Results for Bag-of-Words HMD}
\label{sec:bow-results}

%
%%-------------------
%\begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/7.bow/bag-of-words-results.pdf}\par
%\caption{(Bag-of-words) Detection accuracy and false positive rates for synthetic malware}
%\label{fig:synthetic-malware-bow}
%\end{figure}
%%-------------------
%

%We performed extensive evaluation of the Bag-of-Word model, and report here
%its capabilities in the detection of synthetic malware embedded in Android
%apps. 
%Different from the online detection in the Markov model,


\ignore{In these experiments, we use the given TTD window to
divide the traces from each application, including both the hour-long
trace under normal execution and the shorter traces with malicious,
along the time dimension into a set of non-overlapping small traces,
each of which has length TTD. We view them as independent observations
and construct a bag-of-word vector for each of them. Then, we use all
the vectors from the baseline app execution to train the one-class
SVM, and perform detection on both the normal traces and the traces
with malware workload.} 

Our bag-of-words model results show that HMD models should be chosen specific
to each application, and that there is an opportunity to apply ensemble methods
to boost detection rates.

Bag-of-words model treats program phases as words and a (configurable) {\em
Time-to-Detection (TTD)} window as a document.  We experimented with a range of
TTDs and found TTD = 1.5 seconds to yield good results (in
Figure~\ref{fig:synthetic-SVM-heat-map}).  
We parameterize the one-class SVM so that it has around
20\% percent of false positives. 

\ignore{
The `\%' column reports true
positives, i.e. the correctly identified TTD windows, from a total
`\#TTD' time windows.
%The corresponding TTD column shows the total number of TTD windows in the
%corresponding experiment. For examples, in the case of 
For example, Amazon app has 930 TTD windows where malware exfiltrates photos
("Pictures" line), and only 79\% of them were identified correctly. 
}
%Due to space constraints, we present results
%only for the five apps.

%We use a Gaussian kernel with bandwidth $g$ for the one-class SVM, and
%set the $\nu$ parameter for 

%We use a grid-search approach to
%find the bandwidth ($g$) and $\nu$ to give us the best true positive rate on malicious
%activities with around 20\% of false positives. 
Figure~\ref{fig:synthetic-SVM-heat-map} shows that the bag-of-words 
model: 1) achieves surprisingly high true positive rate for dynamic, compute intensive apps
such as  Angry Birds 
(99.9\%), CNN (84\%), Zombie WorldWar (93\%), and Google Translate (92.4\%) 
with around 20\% false positive rate; 
and 2) achieves around 80\% true positive rate for both Amazon and Sana with
around 20\% of false positive rate. 
%We could not control the error rate for TuneInRadio; nevertheless, our method
%achieves 90\% true positive rate with 38\% false positive rate for TuneInRadio
%app.
Interestingly, the Markov model works significantly better than bag-of-words 
for TuneIn Radio -- with a 10\% FP: 90\% TP rate compared to 38\%FP: 90\% TP
rate respectively -- but performs significantly worse on apps like Angry Birds.
%Overall, 
%In comparison to the Markov model, 
%the bag-of-words achieves a higher true positive rate but at the cost of a
%18\%--38\% false positive rate.
%This example shows that some models maybe more adequate for certain categories
%of app. 
In summary, a deployed HMD will benefit from choosing the models that work best
for each application, but due to their different TP:FP 
operating points, will also benefit from
using boosting algorithms in machine learning~\cite{schapire2012boosting}.



%-------------------
\begin{figure}[tbp]
%\vspace{-0.2in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/4.reflection/phase_tp_vs_phase_fp.pdf}\par
\caption{(Markov model) Effect of obfuscation and encryption on detection rate: interestingly, malware becomes more distinct compared to baseline
benign app.}
\label{fig:reflection}
\end{figure}
%-------------------


\subsection{Composition with Static Analyses}
\label{sec:reflection}

Reflection is a powerful method for writing malware that 
evades static program analysis tools used in App Stores
today~\cite{Livshits_Reflection_Java}, \cite{evade-bouncer}. Interestingly,
we show that malware that uses
reflection to obfuscate its static program paths
in turn worsens its dynamic hardware signals, and 
improves HMDs detection rates.
 
Java methods invoked via reflection are
resolved at runtime, making it hard for static code analysis to
understand the program's semantics.
%
At the same time, reflection alone is not  sufficient --
all strings in the code must also be encrypted, 
otherwise the invoked method or a set of possible
methods might be resolved statically. 
%
We augmented our synthetic malware with
reflection and encryption similar to Geinimi.a\textquotesingle s
implementation. 


Static analysis of our malware does not reveal any API
methods that might raise alarms --
we tested this using the
Virustotal online service which ran 38 antiviruses on our apk without
raising any warnings. 

%The result of running our malware detector on the 
Figure~\ref{fig:reflection} shows results of using HMDs on the 66 synthetic
malware samples augmented with reflection and encryption, and embedded into
AngryBirds, Sana, and TuneInRadio.
%
%We deliberately show the results in the "raw" format, i.e. in terms of the raw
%phase windows that the Markov model operate on, because they more accurately
%characterize malware detectability.  
We see that in Angry Birds and Sana the detection rate of the malware that uses
both reflection and encryption is significantly higher because reflection and
encryption are computationally intensive and disturb the trace of the benign
parent app (i.e., more than the same malware without reflection and
encryption).  We do not see the same trend for TuneInRadio because its
detection rate was already quite high, so the additional impact of reflection
on TuneIn Radio stays within the noise margin. 
We conclude that HMDs complement current static analyses and can
%and static analyses can together present 
potentially reduce the pressure on
computationally intensive dynamic analyses with larger trusted code
base~\cite{taintdroid}.

%reflection and accompanying encryption 
%increase malware
%detectability by our malware detection scheme in the average case.








%%%%%%%%%%%%%%%%%%%  GRAVEYARD %%%%%%%%%%%%%%

\ignore{

We performed extensive evaluation of both the Markov model and the
bag-of-words (BoW) model. The final performance of the detector is 
reported the results as the percantage of detected 
malware samples versus the number of misclassified 30-sec windows. Some 
intermediate results whose goal is to analyze some technical properties 
of Markov model-based detector are shown in terms of phase windows.
%Due to space limitation, we mainly report here our
%findings with Markov model, briefly summarize 
%the results of the BoW model. %, and at the end present a 
%boosting algorithm that can efficiently combine our classifiers to improve 
%detection accuracy.
%
We tune the parameters for our models on a per-app basis in all experiments
throughout the paper.


\subsection{Diversity of Baseline Apps}
\label{ben-app-diversity}


%For comprehensive evaluation of the proposed approach we chose three apps from
%out test suite: 
%%For comprehensive evaluation of the proposed approach, we chose three apps from
%%out test suite: Angry Birds, Sana, and TuneIn Radio. These apps represent three
%%fundamental categories in our classification of Android programs:
%%computationally intensive, event-driven, and network-intensive apps. To prove
%%that the chosen apps exhibit completely different dynamic behavior, we applied

We first investigated whether the nine baseline applications that we had chosen are
sufficiently diverse. To quantitatively analyze the diversity of the apps, 
we applied Principal Component Analysis (PCA) to the 
instruction mix to visualize the
distribution of the apps in a two-dimensional space,  
as well as a behavioral comparison of apps in the feature space 
using the Markov model (Figure~\ref{fig:baseline-diff}). 

The PCA method projects the apps' instruction mix 
on the first two principal components that retain 90.77\% of variability in the data. We see that the 
apps are evenly scattered over the region, and they do not form any clusters. Therefore, 
the programs we have chosen as underlying benign apps are diverse with respect to their 
low-level characteristics.

The second method compares apps at a higher level than PCA. Due to space limitation, 
we present results of this comparison among only three apps: AngryBirds, Sana, and TuneInRadio (Figure~\ref{fig:baseline-diff}), 
because they represent the three broad categories of Android apps: computationally intensive, 
event-driven, and network intensive apps.
When comparing the apps, we treated one of them as baseline and the
remaining two apps as novel ones. Thus, we used the model built for the
baseline app to measure the divergence of the dynamic behavior of the other apps.
Results are reported in
Figure~\ref{fig:baseline-diff} with the following axis: percentage of the true
positives versus percentage of the false positives in terms of phase-level
windows, which is the same as the {\em state\_window} we defined
in sec.~\ref{sub:representation}.  The number of true positives characterizes how
the traces of the novel apps are different from the traces of the selected
baseline app. The resulting step-like curves highlight the inherent dissimilarity
between the apps, and justifies our decision on choosing representative apps in
our test suite. We also see that the dissimilarity measured this way is
not symmetric, which follows from the probabilistic nature of the Markov
models and the noise in the input data. 
Interestingly, this experiment also shows that
it is relatively easy to differentiate the apps using their counter traces.
%Differentiating repackaged apps from their own baseline app, however, is a much
%more challenging proposition (Figure~\ref{fig:pca_all}). %ref to the joint PCA plot
 %(as the false positive results for repackaged
%malware demonstrate). 

\ignore{
%%%%%%%%%%%%%
\subsection{Checking ML Pipeline on Prior-work Dataset}

Compare results to Columbia malware dataset. TODO: remove subsection if not complete
}


%%%%%%%%%%%%%
\ignore{
\subsection{Detecting Existing Malware}

%One point we make in this paper is that our ML models work fine on real
%malware samples. To prove this statement, 

%Known malware samples were not written  \name's anomaly detector.
%%-------------------
%\begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/PLOTS_FINAL/7.time-window/apk_tp_vs_30_sec_time_window.pdf}\par
%\caption{(Markov model) Detection accuracy of synthetic malware reported in terms of 
%discovered malicious APKs (TP axis) versus the number of false positives measured over 30-sec time windows (FP axis).}
%\label{fig:synthetic-malware-apk}
%\end{figure}
%
%\begin{figure*}[t]
%  \subfloat[Angry Birds (AB)]{
%    \label{fig:ab-real}
%    \includegraphics[width=.245\textwidth]{figs/PLOTS_FINAL/1.real-malware/AB-phase_tp_vs_phase_fp.pdf}
%  }
%  \subfloat[Sana]{
%    \label{fig:sana-real}
%    \includegraphics[width=.245\textwidth]{figs/PLOTS_FINAL/1.real-malware/Sana-phase_tp_vs_phase_fp.pdf}
%  }
%  \subfloat[Radio]{
%    \label{fig:radio-real}
%    \includegraphics[width=.245\textwidth]{figs/PLOTS_FINAL/1.real-malware/Radio-phase_tp_vs_phase_fp.pdf}
%  }
%  \subfloat[Monkey Jump]{
%    \label{fig:geinimi-real}
%    \includegraphics[width=.245\textwidth]{figs/PLOTS_FINAL/1.real-malware/Geinimi-phase_tp_vs_phase_fp.pdf}
%  }
%  \caption{(Markov model) Accuracy on detecting real malware repackaged into other apps, reported as the number 
%  of true positives versus the number of false positives computed in the phase-window scale.
%  %\lluis{Lines should only show the malware's name.}
%  }
%   \label{fig:real-malware}
%\end{figure*}
%
%-------------------
%-------------------
\begin{figure}[tbp]
\vspace{-0.1in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/5.ttd/signatures.pdf}\par
\caption{(Markov model) Time to detection and signature sizes for each baseline app.}
\label{fig:time-to-detect}
\end{figure}
%-------------------

%-------------------
\begin{figure}[tbp]
\vspace{-0.1in}
   \centering
   \includegraphics[width=0.45\textwidth]{figs/7.bow/bag-of-words-results.pdf}\par
\caption{(bag-of-words) Detection accuracy and false positive rates for synthetic malware}
\label{fig:synthetic-malware-bow}
\end{figure}
%-------------------

\mikhail{The goal of the HACS' evaluation on the existing malware is to understand 
how the underlying Android apps affect detection of the real malware samples.
}
We evaluated \name using representative instances of real malware chosen
from three malware categories (Sec.~\ref{sec:malware-gen}): information
stealers (Geinimi.a, Roidsec), network-intensive malware (click fraud), and
computationally intensive malware (md5 cracker).  We obtained an instance
of Geinimi.a that was already repackaged into the game MonkeyJump2. We
reverse-engineered all other malware samples and embedded them into Angry
Birds, Sana and TuneIn Radio \mikhail{that represent three different categories 
of the benign apps (Sec.~\ref{ben-app-diversity})}. 
Md5 cracker was not originally positioned as a
malware; it is freely available through Google Play market. 

\ignore{At the time of 
conducting experiments, we did not observe computationally intensive malware 
on the Android platform in the world. That is why we treated 
md5 cracker as malicious app and repackaged it into other benign apps.} 
In total,
we conducted 10 experiments with real malware samples %(Figure~\ref{fig:real-malware}),
which demonstrate the capability of \name in detecting different
categories of malware embedded in inherently different
types of the apps.

\mikhail{To visualize detection ability of the proposed ML algorithms in 
the case of existing malware, we present the ROC curves (Figure~\ref{fig:real-malware}) 
for the Markov model. The ROC curves illustrate performance of the Markov 
model in terms of false and true positives.
}

Comparing the click fraud’s detectability relative to other malware types, we
see that click fraud has higher chances of being detected within network-light
apps (Angry Birds and Sana). However, we notice that detectability
growth rate of click fraud is very low in the interval [3\%, 10\%]. Thus,
we think that it can partially hide itself within the network-intensive app
(TuneIn Radio). 

The other malware, Roidsec, demonstrates the worst detectability in all three
experiments because its activity bursts are separated by dormancy intervals
whose length is larger than the length of activity intervals. In spite of
stealing many types of sensitive data, only in two cases it exhibits
computationally intensive behavior: stealing contacts and text messages. In the
other cases, Roidsec accesses private data without incurring noticeable
overhead (e.g., Wi-Fi status, ROM/SDcard info, etc.) and uploads it to the C\&C
server. %\mikhail{Roidsec exhibits the lowest detectability in our experiments.}
%After averaging the detectability of individual malicious operations
%carried out by Roidsec, we obtained the lowest detectability on average. 

The detection rate of the third malware sample, md5 cracker, mostly lies between
the detectability of click fraud and roidsec, if looked at a reasonable
false-positive interval [0\%, 15\%].  This is because it is more computationally
intensive than roidsec, but not as much as click fraud. Md5 cracker slowly
brute forces md5 hashes using just a single thread. Due to such ineffective
nature, it does not impact the traces of AngryBirds and Sana. However, md5
cracker demonstrates good detectability in the case of TuneInRadio, which can
be explained by noticing a regular structure of TuneInRadio traces. TuneInRadio
activity occurs within evenly spaced bursts, and they resemble the positive
part of $sin(x)$ function. This fact may be a result of buffering data and
processing data in chunks. Between processing chunks of the incoming data,
TuneInRadio’s activity reaches very low values. When md5 cracker overlaps
TuneInRadio, it significantly changes the structure of TuneInRadio’s trace.
%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/7.bow/bow_roc.eps}\par
\caption{(Markov model) Malware samples repackaged in AngryBirds, Sana and 
	TuneInRadio that are undetected by our pipeline. All remaining 
	synthetic malware repackaged in these 3 apps can be detected reliably.}
\label{fig:synthetic-undetected}
\end{figure}
%-------------------

%-------------------


%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/7.bow/bag-of-words-results.pdf}\par
\caption{(bag-of-words) Detection accuracy and false positive rates for synthetic malware}
\label{fig:synthetic-malware-bow}
\end{figure}
%-------------------

\ignore{
%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/bag-of-words-results-1.pdf}\par
\caption{(bag-of-words) Detection accuracy and false positive rates for synthetic malware}
\label{fig:synthetic-malware-bow-1}
\end{figure}
%-------------------
%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/bag-of-words-results-2.pdf}\par
\caption{(bag-of-words) Detection accuracy and false positive rates for synthetic malware}
\label{fig:synthetic-malware-bow-2}
\end{figure}
%-------------------
}
The most complex sample in our dataset is Geinimi.a; it mainly functions as
infostealer, but also includes other functionality (e.g., the ability to
install third-party apps) and thus open doors for other attacks. 
We conducted two series of experiments for Geinimi.a sample that is 
already repackaged into MonkeyJump2 game: MonkeyJump2 with its malicious payload enabled and
disabled. To disable Geinimi.a, we reverse-engineered the apk \mikhail{and commented out 
the code that launches malicious functionality}, then compiled the app again. Due to computationally intensive
behavior of MonkeyJump2 game, we did not achieve 100\% detection rate as in the
case with other malware samples (Figure~\ref{fig:real-malware}). Our results
obtained for Geinimi.a malware are similar to the results for AngryBirds with
embedded Roidsec: neither allows a high level of
detectability.

%then compiled the app again. Because of the computationally intensive behavior of
%the MonkeyJump2 game, we did not achieve a 100\% detection rate as in the case with
%other malware samples (Figure \ref{fig:geinimi-real}). Our results obtained for
%Geinimi.a malware are similar to the results for AngryBirds with embedded
%Roidsec (Figure \ref{fig:ab-real}): neither allows a high level of detectability.
%%% 31316047eecf4886b75b95e3c214a04546cbcd41
}

%%%%%%%%%%%%%
\subsection{Detecting Synthetic Malware}

%-----------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/6.heat_map/heat_map.pdf}\par
\caption{(Markov model) Detectability of synthetic malware: the size of malicious payload grows from
the top to the bottom, and the the amount of delay increases
from the left to the right.}
\label{fig:synthetic-MM-heat-map}
\end{figure}
%-------------------
%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/apk-30-sec.eps}\par
\caption{(Markov model) Malware-level true positive versus 30-sec false positives: detection accuracy for synthetic malware.}
\label{fig:synthetic-malware-phase}
\end{figure}

\ignore{and avoid time-consuming
reverse-engineering of real malware samples, based on the analysis of existing
malware we developed a synthetic malware that adjusts its intensity by loading
configuration parameters from a supplied file.} 

\mikhail{We used synthetic malware developed in-house to evaluate our Andorid 
malware detector and analyze which conditions that cause our malware detection scheme to break. 
To analyze the breakdown conditions, we fine-tuned the intensity of malicious activities within the malware.
It is worth mentioning that we could not find existing malware samples on Android platform 
that include an embedded mechanism for controlling their intensity. 
}

%with high degree of adjustable parameters in order to vary their intensity. 
To conduct experiments with malicious activities at different
intensity levels, we generated 66 malware intensity configurations that specify the malware parameters
for seven types of malware. \mikhail{The summary of the key malware 
parameters is presented in the Figure~\ref{fig:synthetic-malware}. Choosing 
malware parameters in a smart way let us cover the large parameter space and
within that paramater space, detection rate varies from good to bad.
} 
We then conducted 66 experiments with each of
the 9 benign apps in our evaluation. \mikhail{ In the table~\ref{fig:baseline-apps} we 
describe the user input that we used to exercise the apps and the other 
profiling characteristics.
}

 
%we prepared 66 configuration files
%describing 7 types of malware with different parameter settings
%(Figure~\ref{fig:synthetic-malware}).  We conducted 66 experiments with each of
%the 9 benign apps in our test set (Figure~\ref{fig:baseline-apps}). 
%We specifically
%included a range of malware parameters to cover very small perturbation 
%of a benign app to a (likely) larger perturbation 
%will (likely) cause the detector to fail as well succeed. Hence,

\mikhail{
We first give some intuition into how our Markov model detects malware. Figure~\ref{fig:ab} 
shows detection results for the three variations of the click fraud malware inserted 
into Angry Birds that differ only by intensity, from highest intensity (left Figure) to lowest (right Figure). 
Angry Bird's benign traces are 
shown by the light gray color, and malicious traces are black. Every point of these 
curves represents the joint probability (vertical axes) of several consecutive phase\_windows 
(sec.~\ref{Sec:detect-markov}). The horizontal axes is time.
The malicious traces are less probable than benign ones; their probability mostly lies outside of two standard deviations 
from the mean of the benign traces. The benign traces have occasional spikes of decreased probability that 
are also two standard deviations from the mean. These spikes result in false positives during malware detection, but are localized in time.
Further, when reducing malware intensity 
benign and malware traces start overlapping more, leading to poor detectability, i.e.  
higher false positive rate. 
}

Second, we analyzed in details how our malware detector works on all $9*66=594$ malware 
samples that we have in our collection. The results for the Markov model based detector are shown in the form of a heat 
map in Figure~\ref{fig:synthetic-MM-heat-map}. Malware categories (file stealer, contact stealer and etc) 
are shown on the left-hand side of the table, and data in columns correspond to a particular app.
The intensity of the color - from light blue up to dark blue - corresponds to the detectability level,
which is computed as the number of raised alarms versus the the total number of alarms that
could be raised. All the results are show for the FP rate 20-25\%.

Within each cell corresponding to an app and a particular malware category, the size of malicious 
payload grows from the top to the bottom, and the the amount of delay increases from the left to the right.
As we mentioned before, we have three levels of delay: zero, medium and high (they are denoted by the 
symbols "N", "M" and "H" at the bottom of the heat map). The small white cells with "X" symbol in them 
mean that we did not conduct a corresponding experiment. When testing the ID+GPS stealer, we use only two 
type of delays - zero and medium - because even zero delay makes detection really hard due to negligible
computational overhead. The parameters on payload size are consistent with the table in Figure~\ref{fig:baseline-apps}.

One of the goals of our experiments was to find out how payload size and frequency can affect detectability. Spot 1 
in Figure~\ref{fig:synthetic-MM-heat-map} sheds light onto the correlation between payload size and detectability. We assume 
that larger malicious payload (e.g. uploading to a remote server more pictures or contact) makes malware
more visible to the detector. Further, slowing down the malware by inserting the artificial delays,
shown in Spot 2 of Figure~\ref{fig:synthetic-MM-heat-map},
may reduce detectability, but this may not be a very reliable method of escape from a malware detector due to 
runtime optimizations. From the heat map, we do not see that this is consistent across all apps and malware categories.

As we mentioned before, the prupose of varying the intensity of malicious payloads is to find when our detector breaks.
Spot 3 in Figure~\ref{fig:synthetic-MM-heat-map} shows that brute-forcing a SHA1 hash with the limit of 10K iterations
is barely noticeable when Sana is executed. 
Despite the light-weight nature of Sana app, it exhibits bursty behavior which might explain why short-time malware does not 
stand out.

To evaluate overall performance of the detector, we generated traditional ROC curves (Figure~\ref{fig:synthetic-malware-phase}).
The ROC curves show the percentage of detected malware samples (TP rate) versus the number of false alarms raised on per 
30-sec window basis. In other words, if an alarm is raised within a 30-sec window, the entire window is considered to 
be malicious by our malware detection scheme.

The ROC curves are meant for the pair-wise comparison of the detection rates between the separate apps. 
Note that low detection accuracy does not imply inherent flaws 
in our machine learning pipelines because we intentionally included undetectable 
samples in our test suite and did not try to skew the detection 
results in our favor.

\ignore{
Second, we summarize hard to detect malware samples in
Figure~\ref{fig:synthetic-undetected}. Only 20 samples out of 66*3 = 198 remain
undetected, and the combination of payload to the baseline app offer insights
into what can and what cannot be detected. 

For instance, Angry Birds is a
computationally intensive game that allows malware to steal 400 SMSs at a time,
whereas TuneIn Radio is much more sensitive -- even stealing a single photo or
25 SMSs triggers a true positive. \mikhail{The user-driven app, Sana, occupies the position 
between two extremities, Angry Birds and TuneIn Radio.}
}
\ignore{
\mikhail{Third, we compute the aggregated statistics over the generated 
set of the malware samples. The ROC curves presented on the Figure~\ref{fig:synthetic-malware-phase} are meant 
to be used for the pair-wise comparison of the detection rates between the separate apps. 
We should highlight the fact that low detection accuracy does not imply inherent flaws 
in our machine learning pipelines because we intentionally included undetectable 
samples in our test suite. And we did not try to skew the detection 
results in our favor.
}
}

Overall, we find that our Markov model approch to malware detection (Figure~\ref{fig:synthetic-malware-phase}) 
works best for the apps with predictable
(as in simple or regular) behavior. The top three curves, corresponding to the Amazon, Firefox and
TuneInRadio apps, have ~17\% FP vs ~88\% TP.
Unlike the other apps, Amazon does not exhibit complex dynamic
behavior. While TuneInRadio has complex behavior, it is highly regular and
looks like the $f(x) = mod(sin (x))$ function. In these apps, even small perturbations can
be detected very well.  

While one may think that CNN is conceptually similar to
Amazon, we do not achieve as good detection for CNN as for Amazon.
This may be because CNN's dynamic behavior varies quite a bit: CNN can provide text news, show
pictures and play videos, display static and animated ads. 
CNN and the game Zombie WorldWar are worst in terms of the scalability of the results, i.e.
allowing for more false positives improves their malware detectability insignificantly. 
Malware embedded into these two apps manage to hide itself much better than within the other apps.


Detection rates of the rest apps are grouped together around Sana's curve. One
may expect that Sana should leave a highly predictable signature due to the
simplicity of its user interface. However, this is not the case as user events
cause short and sharp spikes within the traces, which could not be reliably captured
by the Markov model. For most applications, the Markov model can reliably detect
from 30\% to 90\% of malware samples while not exceeding a 10\% false
positive rate.

\ignore {
\mikhail{Here we make a transition from defining a false positive as a 
misclassified phase\_window (50ms -- 150 ms) to a misclassified 30-sec 
window. The detector's performance changes significantly.
}
%We also experiment with transition from near real-time detection to more coarse
%grained time scale. 
The Figure~\ref{fig:synthetic-malware-apk} shows apk-level true
positive rate (the number of detected malicious apks over the total number of
malicious apks) vs the false positive rate computed over the 30-sec time
windows. We see that the detection to false positive ratio is much better
%area under the  curve is higher in this case than
in the case v. when we measure detection in terms of phase windows
(Figure~\ref{fig:synthetic-malware-phase}). This finding means that detection
improves given a longer time scale. However, false positives tend to cluster
together so that the rate is better with 30s windows than at the phase level.
}
\ignore{
\begin{comment}
We also experiment with transition from near real-time detection to more coarse
grained time scale. Figure~\ref{fig:synthetic-malware-apk} shows apk-level true
positive rate (the number of detected malicious apks over the total number of
malicious apks) vs the false positive rate computed over the 30-sec time
windows. We see that the detection to false positive ratio is much better
%area under the  curve is higher in this case than
in the case v. when we measure detection in terms of phase windows
(Figure~\ref{fig:synthetic-malware-phase}). This finding means that detection
improves given a longer time scale. However, false postives tend to cluster
together so that the rate is better with 30s windows than at the phase level.
\end{comment}
}
% coarser scale
%we choose, the more accurate results we cam obtain 

%(results consistent with
%Demme et al.~\cite{perf_counters_2013}).



\ignore{
%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/PLOTS/2.b.variation-of-time-window-size/apk_tp_vs_apk_fp.pdf}\par
\caption{Detection accuracy v. warning time parameter (in number of phase windows below detection threshold)}
\label{fig:synthetic-malware}
\end{figure}
%-------------------
}

%%%%%%%%%%%%%


%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/4.reflection/phase_tp_vs_phase_fp.pdf}\par
\caption{(Markov model) Effect of obfuscation and encryption on detection rate: interestingly, malware becomes more distinct compared to baseline
benign app.}
\label{fig:reflection}
\end{figure}
%-------------------
\subsection{Reflection}
\label{sec:reflection}
Reflection is a powerful method for writing malicious code that is meant to
escape from static code analyzers. \mikhail{Here we analyze how reflection 
affect the detection rate.}

Java methods invoked via reflection are
resolved at runtime, making it hard for static code analysis to
understand the program's semantics. At the same time, pure reflection is not
enough to protect against static analysis of the code --- it must be accompanied
by encryption of strings, otherwise the invoked method or a set of possible
methods might be resolved statically. We augmented our synthetic malware with
reflection and encryption in a way that is similar to Geinimi.a’s
implementation. Static analysis of our synthetic code does not reveal any API
methods that might allow static tools to raise alarms. We checked this using the
virustotal.com online service, which ran 38 antiviruses on our apk, and we did
not receive any warnings. 

The result of running our malware detector on the 66
synthetic malware samples augmented with reflection and encryption, and
embedded into AngryBirds, Sana, and TuneInRadio is shown on the Figure~\ref{fig:reflection}. 
We deliberately show the results in the "raw" format, i.e. in terms of the raw phase windows
that the Markov model operate on, because they more accuretely characterize malware detectability.
We see 
that in the case of AngryBirds and Sana the detection rate of the malware that
uses both reflection and encryption is significantly higher because reflection
and encryption are computationally intensive and disturb the trace of a
benign app more than the same malware without reflection and encryption.
We do not see exactly the same trend for TuneInRadio because its basic
detection rate is quite high, so the results with TuneInRadio
stay within the error range. 

We conclude that reflection and accompanying
encryption increase malware detectability by our malware detection scheme in the average case.

\subsection{Parameters of Benign Apps' Signatures }

%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/5.ttd/signatures.pdf}\par
\caption{(Markov model) Time to detection and signature sizes for each baseline app.}
\label{fig:time-to-detect}
\end{figure}
%-------------------



We provide insights into what overhead could a detector based on Markov model
incur on hardware, network and etc. For this purpose we computed the size of 
the signatures describing behavior of the benign apps (Figure~\ref{fig:time-to-detect}). 
They lie in the range from 1212 bytes to 6724 bytes, with an average size of 3.2Kb. 
Such small sizes make storing and transferring signatures extremely fast, and 
their enforcement at runtime is unlikely to cause significant overhead.

The other crucial parameter is the time to detection -- it characterizes how 
fast the system can react to an ongoing threat. We measured this parameter 
by starting our malware detector and malware sample simultaneously. Time 
to detect parameter depends on the number of states in the Markov model, 
the length of phase\_windows and the number of subsequent states to be observed 
before the detector can make a decision.

From the Figure~\ref{fig:time-to-detect} one can see that time to detect 
lies in the range 1280ms to 4400ms, while in most cases it is about 2.5 seconds. 
This means that the system can stop many suspicious activities at the very beginning. 
The detector may miss exfiltrating the first photo (it takes 2.86 sec on average), 
but it is likely to prevent the theft of the second one.

\mikhail{When developing the real-time malware detector, the main tradeoff is time to detection vs. false positive rate.
That is, reducing the time to detect parameter increases the false positive rate because 
the detector must make a decision with only the limited information collected within 
the time to detect window.
}

\subsection{Results for Bag-of-Word Model}

%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/7.bow/bag-of-words-results.pdf}\par
\caption{(bag-of-words) Detection accuracy and false positive rates for synthetic malware}
\label{fig:synthetic-malware-bow}
\end{figure}
%-------------------


We performed extensive evaluation of the Bag-of-Word model, and report here
its capabilities in the detection of synthetic malware embedded in Android
apps. Different from the online detection in the Markov model,
Bag-of-Word model works with a predefined {\em Time-to-Detection
  (TTD)} window. 

\ignore{In the experiments, we use the given TTD window to
divide the traces from each application, including both the hour-long
trace under normal execution and the shorter traces with malicious,
along the time dimension into a set of non-overlapping small traces,
each of which has length TTD. We view them as independent observations
and construct a Bag-of-Word vector for each of them. Then, we use all
the vectors from the baseline app execution to train the one-class
SVM, and perform detection on both the normal traces and the traces
with malware workload.} 

We performed a study for a variety of TTDs, 
and reported in Figure~\ref{fig:synthetic-malware-bow} the results for TTD = 1500 ms. 
The percentage column characterizes the relative number of identified TTD windows. 
The corresponding TTD column shows the total number of TTD windows in the 
corresponding experiment. For examples, in the case of Amazon app we have 930 TTD 
windows where malware exfiltrates photos ("Pictures" line), and only 79\% of them 
were identified correctly. Due to space constraints, we present results only 
for the five apps.

We use a Gaussian kernel with bandwidth $g$ for the one-class SVM, and
set the $\nu$ parameter for the one-class SVM so that it has around
20\% percent of false positives. We use a grid-search approach to
find the $g$ and $\nu$ to give us the best true positive rate on malicious
activities with around 20\% of false positives. 

From Figure~\ref{fig:synthetic-malware-bow}, we see our method: 1) achieves
surprisingly high true positive rate for both AngryBrids (99.9\%) and
Google Translate \\ (92.4\%) apps with around 20\% of false positive rate; 2)
achieves around 80\% true positive rate for both Amazon and Sana with
around 20\% of false positive rate. We could not control
the error rate for TuneInRadio; nevertheless, our
method achieves 90\% true positive rate with 38\% false positive rate
for TuneInRadio app.

\mikhail{In comparison to the Markov model,bag-of-words achieves much higher true 
positive rate at the cost of 18\%--38\% false positive rate. In the case of 
TuneIn Radio, Markov model works significantly better than bag-of-words. 
The former has 10\% FP and 90\% TP, while the latter suffers from 38\%FP and 
90\% TP. This examples shows that some models maybe more adequate for certain 
categories of app. There is an opportunity to apply ensemble methods to use 
multiple models simultaneously.
}

\ignore{
\subsection{Ensemble Methods}
The two machine learning models, Markov chain and BoW, 
demonstrate qualitatively different performance in detecting malicious
activities. While Markov model tends to keep the number of false positives low, 
for most applications it does not achieve high detection rate (Figure 10). On 
the other hand, BoW detects large number of malicious activities, but its false 
positive rate is relative high. To combine the best aspects 
of these two models, we use ensemble method to boost their performance. 

We make two adjustments to the Markov model to make it easy to combine
it with the BoW model. First, we set the length of the phase window
and the size of the detection window in Markov model in a way that the
detection window equals to the Time-To-Detection (TTD) window in BoW
model.  This adjustment slightly decrease the detection rate of Markov
model. Second, we convert the phase-level decision of Markov model 
into TTD-level classification of BoW model. To assign a label to a particular 
TTD window, we apply voting approach to the class labels of the three consecutive 
phases windows \ling{This part is very difficult to understand: 
whose labels are computed over at least all but one phases of the current 
detection window.} 

We use a switch model to perform the ensemble.  Recall that in the BoW 
model we use one-class SVM to find a minimum hypersphere that can
enclose most of the normal observations. When we do ensemble
detection, we mostly rely on the detection result of
BoW model unless points are very close to the SVM hypersphere. When points are 
very close to hypersphere, we use the result of the Markov model. The 
threshold for switching between the two models is empirically determined 
based on multiple experiments. This switch ensemble
method enables us to better capture both the statistical (BoW) and temporal (Markov model) 
properties of the executed code than either of the individual model. 
As a result, we significantly reduce false positive rate while still
achieve high detection rate  for most apps in our data set (Figure~\ref{fig:boosting-table}).

Comparing results of individual models (Figure~\ref{fig:synthetic-malware-phase},~\ref{fig:synthetic-malware-bow}) 
to that of the ensemble model (Figure~\ref{fig:boosting-table}), we see that Amazon's FP 
and TP rates did not change much, the former decreased by 2.5\% and the latter increase by 3\%.
This comes from the way we implemented the ensemble method: it mainly relies on BoW 
model, however the Markov model works far better in this case. In the other cases 
(e.g. AngryBirds, Sana, TuneInradio and etc) we see dramatic improvements in 
terms of the number of FPs. However, the price of this is a little drop of the 
TP rate in some cases (e.g. Sana's TP rated dropped by 4.34\%).

Based on this experiment, we see that it is highly unlikely to find a single model 
that would capture intrinsic properties of all types of applications. Ensemble 
methods can easily increase accuracy of modeling an app's behavior by combining 
the baseline models in different ways.

\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.4\textwidth]{figs/boosting-table.pdf}\par
   \caption{Results of using boosting to reduce the number of FPs and increase the number of TPs.}
   \label{fig:boosting-table}
\end{figure}


\ignore{
\begin{table}[ht] 
\caption{Boosting} % title of Table 
\centering % used for centering table 
\begin{tabular}{c c c c c c} % centered columns (4 columns) 
\hline\hline %inserts double horizontal lines 
Parameter   & Amazon & AngryBirds & GoogleTranslate & Sana & TuneInRadio \\ [0.5ex] % inserts table 
%heading 

\hline % inserts single horizontal line 
TP,~\% & -- & -- & -- & -- & 92.7 \\ % inserting body of the table 
FP,~\% & -- & -- & -- & -- & 9.95 \\ [1ex] % [1ex] adds vertical space 
\hline %inserts single line 
\end{tabular} 
\label{table:boosting} % is used to refer this table in the text 
\end{table}
}


\subsection{Supervised learning}

\ling{I am not sure whether we need this section given that: 1) We
  have the ensemble method to achieve low FP and high TP detection; 
2) the performance of supervised learning is just so so. There are
just too many things in the paper for the review to digest.}

\color{red}
We deliberately preferred unsupervised approach (anomaly detection) 
to supervised one. Supervised algorithms are sensitive to the 
quality of malware training set, i.e. to how malware training set resembles 
the real life. A classifier may be skewed because of the poor quality 
of the training set. 

The number of semantically equivalent code transformations of a malware 
sample is infinite. The use of a few malware samples in the training 
set may not necessarily improve the quality of the model. To support 
this claim, we turned the BoW model into supervised classifier by replacing 
1-class SVM with 2-class SVM. Then, we trained it on 80\% of benign samples 
of a particular app and different amounts of randomly chosen 
malicious samples. In all experiments, the size of malware training set 
was equal to the size of benignware training set. Both benign and malware 
samples not used for training phase were used for testing, and we report 
accuracy of based on the testing the classifier on the previously unseen 
samples (Figure~\ref{fig:supervised-learning}).

We see that the resulting classifier demonstrates adequate performance only 
if it is trained on at least 20-40\% of the malicious samples (the number 
depends on the underlying baseline app).

In the real world scenario, we are unlikely to guarantee that the malicious 
set would represent future malware samples. However, we can model behavior 
of benign apps as thorough as we would like because they do not have an 
intention to hide. Thus, anomaly detection seems to be a better fit for 
Android malware detection than supervised learning approach.

\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.5\textwidth]{figs/PLOTS_FINAL/supervised-learning/supervised-learning.pdf}\par
   \caption{(Supervised learning) Detection accuracy of supervised learning 
algorithm highly depends on the quality of the malware training set.}
  \label{fig:supervised-learning}
\end{figure}

}


\ignore{
\subsection{Analysis of the baseline Malware}
Here we present the aggregate analysis of basic malware types on the 
microarchitectural level, i.e. the number of instructions per one basic 
malicious action and the instruction mix. SMS/Contact in the left column means 
accessing one sms/contact. SHA1 stands for one iteration of pure 
Java implementation of SHA1 password cracker. We see that even ordinary 
actions like SMS~\ref{table:agg-mal-analysis}.
}

\ignore{
\begin{table}[ht] 
\caption{Aggregate analysis of basic malware types} % title of Table 
\centering % used for centering table 
\begin{tabular*}{.5\textwidth}{c c c c c c c c} % centered columns (4 columns) 
\hline\hline %inserts double horizontal lines 
\parbox[c]{0.6cm}{\raggedright Malware Type}  & \parbox[c]{0.6cm}{\raggedright Length, sec} 
 & \parbox[c]{0.6cm}{\raggedright Inst. Count (Million)} & \parbox[c]{0.6cm}{\raggedright Mispred. Branches} &
 \parbox[c]{0.6cm}{\raggedright Imm. Branches} & \parbox[c]{0.6cm}{\raggedright Ind. Branches} &
\parbox[c]{0.6cm}{\raggedright Load/Store Inst.} \\ [0.5ex] % inserts table 
%heading 

\hline % inserts single horizontal line 
SMS & 0.12 & 25.90 & 0.08 & 0.15 & 0.19 & 0.75 & 0.36 \\ % inserting body of the table 
Contact	& 0.36 & 67.80 & 0.04 & 0.21 & 0.24 & 1.00 & 0.41 \\ 
File (photo) & 2.86 & 50.97 & 0.01 & 0.21 & 0.07 & 0.70 & 0.44 \\
Click Fraud & 0.40 & 44.40 & 0.34 & 0.30 & 0.22 & 0.65 & 0.41 \\
SHA1 &	2.8E-5 & 0.02 &	0.02 &	0.22 &	0.20 &	0.58 &	0.37 \\
\parbox[c]{1.0cm}{\raggedright GPS/IDs (textcolor{yellow}{REDO})} & 4 & 49.70 & 0.03 & 0.17 & 0.05 & 0.77 & 0.53 \\[1ex] % [1ex] adds vertical space 
\hline %inserts single line 
\end{tabular*} 
\label{table:agg-mal-analysis} % is used to refer this table in the text 
\end{table}
}

\ignore{
\subsection{Aggregate analysis of our data set}

To demonstrate diversity of the underlying benign applications, we computed 
the dynamic instruction count and the instruction mix (Figure~\ref{fig:benign-agg-stat}). The 
parameters we present here are averaged over multiple runs.

*Radio: 2 threads: we tracked only the main thread, the other thread is more active

*Amazon is really active; thread: n.mShop.android…\#7226

\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.5\textwidth]{figs/PLOTS_FINAL/agg-stat/ut-data-set/benign-agg-stat.pdf}\par
   \caption{Aggregate statistics collected over underlying benign apps. }
   \label{fig:benign-agg-stat}
\end{figure}

The second commonly used method to analyze similarity of the chosen apps is 
PCA analysis (Figure~\ref{fig:pca-ut-benign}). We see that the chosen apps do not form clusters and 
they are well spread out. \ignore{within the set of many other Android apps}.
}
\ignore{
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.5\textwidth]{figs/PLOTS_FINAL/agg-stat/ut-data-set/pca-benign.pdf}\par
   \caption{Benign apps plotted in the PC space.}
   \label{fig:pca-ut-benign}
\end{figure}
}
%\color{black}
\ignore {

\ignore{}
\subsection{Columbia data set}

Our data set is not unique, we obtained a similar data set~\cite{perf_counters_2013} 
and analyzed it. One of the key things we looked at is the length of malware 
execution. For each malware type we summed up all records in the data set 
regardless of training/testing partition. According to Demme et al.~\cite{perf_counters_2013}, 
some samples were executed several times, but we treat all executions as one 
because we do not have information how many times every malicious sample 
was actually executed. Also, we did experiments on the board equipped 
with ARM A15 CPU running at up to 2.5GHz \ref{http://www.arm.com/products/processors/cortex-a/cortex-a15.php}, 
while Demme et al.~\cite{perf_counters_2013} ran malware samples on OMAP4460 
dev. board equipped with ARM A9 CPU running at 1GHz+. Because of using 
much faster and more advanced CPU, our average execution times of 
individual malicious activities shown in the previous section would 
be greater if we tested on OMAP4460 board. Thus, the analysis we 
present here is significantly skewed in the favor of \cite{perf_counters_2013} 
data set. In the \cite{} data set, the time is measured in cycles; when 
we converted cycles into seconds, we assumed 1GHz frequency.

The first thing we did is we plotted the distribution of traces’ length (Figure ~\ref{fig:columbia-benign-CDF}). 
We see that malware execution times are extremely short. In the testing 
environment~\cite{perf_counters_2013},  20\% of malware were tested for 
less than a second, 56\% - less than 10 sec. We assume that common malicious 
payload was not executed in most cases. The total length of all benign traces in 
~\cite{perf_counters_2013} data set is 1h 29 min, malicious traces - 58 min, 
this  is one order of magnitude less than the analogues parameters of our data 
set.Due to space limitation, here we present a brief analysis of 2 
randomly chosen malware samples.

\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.5\textwidth]{figs/PLOTS_FINAL/agg-stat/columbia-data-set/benign-CDF.pdf}\par
   \caption{(Columbia data set). CDF of the benign apps' lengths.}
   \label{fig:columbia-benign-CDF}
\end{figure}



%%%%%%%%%%%%%
\subsection{Experiments on an Alternate Platform}

%-------------------
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.4\textwidth]{figs/PLOTS_FINAL/A1-OMAP5-AngryBirds/phase_tp_vs_phase_fp.pdf}\par
   \caption{(Markov model) Detection accuracy on Samsung Arndale v TI OMAP5432 platform (synthetic malware in Angry Birds). The OMAP
board uses wired network which leads to faster payload execution and a more anomalous compute profile.}
   \label{fig:alternate-platform}
\end{figure}
%-------------------

We also repeated 66 experiments with the synthetic malware injected into
Angry Birds on the other development board, TI OMAP5432, to confirm that our
approach has no implicit hardware dependencies. For this experiment we used the
synthetic malware augmented with reflection and encryption. We
see that the same malware is far more detectable on OMAP5432 board (Figure~\ref{fig:alternate-platform}). We 
found that this effect comes from the speed of the
network connection: OMAP5432 has only high speed Ethernet port, while Arndale
board relies on WiFi connection. Using the Ethernet connection, malware
communicates with its C\&C faster and thus its payload is executed much faster
avoiding blocks on network access and leaving more detectable fingerprint.

%Unfortunately, OMAP5432 does not have WiFi module, so we were no able to
%precisely characterize effects of the speed of a network connection on malware
%detectability.
}

}


==> stdarch.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
% Different font in captions
%\newcommand{\captionfonts}{\small\bf}
\newcommand{\captionfonts}{\small\em\bf}
\makeatletter  % Allow the use of @ in command names
\long\def\@makecaption#1#2{%
  %%\vskip\abovecaptionskip
  \sbox\@tempboxa{{\captionfonts #1: #2}}%
  \ifdim \wd\@tempboxa >\hsize
    {\captionfonts #1: #2\par}
  \else
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  %%\vskip\belowcaptionskip
  }
\makeatother   % Cancel the effect of \makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Compress the heck out of figure gaps
\parskip=0.04in
\floatsep=0.01in
\textfloatsep=0.02in
\dbltextfloatsep=0.02in
\dblfloatsep=0.02in


==> story.tex <==
* 








Title: Evaluating Hardware-based Malware Detectors
         Under Realistic, Adversarial Conditions 


Intro:

* malware!

* Behavioral v. provable/permissions: trusted app get compromised.

* hardware detectors.

* No exploits; only Payloads (ptr to motivation)
   - Configuration errors: File manager apps vulnerable -- wallpaper steals data. Applock. Evernote.
   - Vulnerability in code signing: FakeID attacks, Masterkey, Stolen keys
   - Webview attacks: Same Origin Policy bypass. Browser itself!
   - Phishing: snoopwall

   Diagram mapping Trojans, backdoors, exploits, .... to info stealers, net nodes, and compute nodes.

* Don't run

* Benignware exe

* Adapt

Contributions:
  - taxonomy.
  - benchmark suite: representative real + synth. all running. GOAL: find breaking point. Assume it works beyond.
  - record and replay
  - analysis techniques: signature + anomaly.
  - insights.
------------

Evaluation:
-----------
* did malware really run? -- geinimi
* android v. desktop?
* how mobile different from desktop
Diversity of malware:
   - one malware has many signatures: eg., geinimi!

Encryption:
   - SSL for attacks


Realistic:
   - malware executes

   - benign apps are diverse and used realistically

   - the underlying device is primed with real data, with noise due to UI, middleware, network, etc.


Adversarial
   - malware can adapt payload

   - malware hides behind favorable benign apps.
      = compare with baseline apps

Insights we want:
   - which payload:app combination is detectable? (lies at the boundary)

   - did we get lucky with an ML algo? or is the signal intrinsic to dataset

   - does code obfuscation affect detection? (comparison with existing software-level detectors)
      - benefit of 'why' or understanding payload?


Motivation section
   - run a few of the samples referred in Demme paper.
   - run desktop samples. difference from mobile malware?
   - malware with and without benignware in the background
   - make a figure for many ways to get payloads in --> without exploits --> can I detect payloads.


v. Hardware implementations:
   - mobile malware do not require new hardware. Lossy performance counters are sufficient to detect payloads.
      - Our analysis is efficient even if new hardware is added.
   - lightweight user trace collection 

* ml algorithms in a figure
   - intuition for both


* malware classification
   - summarize prior classifications into malware family names, into non-disjoint categories (marble sec)


* Conclusion
   - why is malware research an arms race? Most defenses are evaluated on existing or older malware. But malware adapts.
     By evaluating ours and existing behavioral detection tools against a diverse, representative workload, we put them to test
     against an adaptive adversary.


==> threat-deploy.tex <==
%\ignore{
%%---------------------------------
%\begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.4\textwidth]{figs/system-overview-3.pdf}\par
%\caption{Proposed system to construct computational signatures of
%{\em benign apps} and use them to test against signatures of 
%malware. Malware is allowed to adapt to avoid detection.}
%\label{fig:deploy}
%\end{figure}
%%---------------------------------
%}

As a complement to offline analyses,
we consider a system that has two components.  On the server side,
a platform provider (e.g., Google) executes benign and/or malware 
applications using test and real
user inputs, measures performance counters, and creates a database of
computational models.
%
%The platform provider then attaches the signature to each application in the
%app-store. 
On client devices, a light-weight system service samples performance
counters to create run-time traces from applications, and compares each run-time
trace to database entries either on the device or the server. 

The database can contain either a black-list (of malware
executions~\cite{perf_counters_2013}) or a white-list (of benign executions~\cite{anomaly-detector-columbia-raid}).
%
In a black-list analysis, the system has to compare each run-time trace with the
entire malware database looking for a possible match. 
%
In a white-list analysis, each run-time trace purports to belong to a specific
app -- hence only the app's signature needs to be matched.  
%
If malware is detected, the system raises a signal to alert the user and/or
the system. The server will further refine its database using
traces uploaded by clients. 

One line of HMD research focuses on {\em desktop} malware which has 
very different characteristics compared to mobile malware.
Ozsoy et al.~\cite{map} extended this technique to use custom
hardware signals and hardware-accelerated classifiers and used
off-the-shelf desktop malware to evaluate their HMD with 90\% true positive
and 6\% false positive rates.
Tang et al.~\cite{anomaly-detector-columbia-raid} present
a white-list (anomaly) detector for desktop malware and evaluate using 
2 benign programs and 3 exploits, achieving 99\% detection accuracy for less
than 1\% false positives.

To understand differences between Android malware we study the Windows malware
used in studies above, comparing 20 Windows malware samples to 20 benign
programs such as pdfviewer, calculator, filetransfer, resizer, screensaver,
etc.
%
We find that Windows malware executed an average of $\sim$60K system calls within 10
minutes v. only 2.5K for benignware. RegSetValue, the system call used to
modify Windows registry, is invoked 820 times by malware and only 72 times by
benignware.  Further, malware spawns 182 processes/threads on average
while benignware spawns fewer than 30.
%
Windows malware have historically targeted gaining control of the machine
whereas Android malware rarely attempt system-level exploits. We discuss unique
aspects of mobile malware further in Section~\ref{sec:mobile-uniq}.

%, we discuss how Android malware propagation methods
%that result in much smaller differences between malware and benign executions.

The closest related HMD work to ours is by Demme et
al.~\cite{perf_counters_2013}, where the authors present a supervised learning
HMD that compares off-the-shelf Android malware to arbitrary benign apps,
yielding an 80:20 true positive to false positive ratio.  However, this
methodology of using off-the-shelf malware and comparing it to arbitary benign
apps can lead to erroneous conclusions, as we discuss next.  

%The above projects, as also future work in HMDs, can benefit significantly
%from the methodology and metrics defined in this paper.

%\todo{move this to impl}
%Note that for prototyping purposes, existing hardware limits
%us to using 6 performance counters at a time and to using development boards
%instead of mobile phones.

%\parbold{Threat Model.} 
\ignore{
We want to use computational signatures to expose
malicious programs when they execute their payload on a mobile device. We
trust the underlying operating system and hardware of the mobile platform, and
intend \name to be an anomaly detector that complements a permissions-based
access control model (as implemented on Android and iPhones). 

One major entry point for malware is user error. Users are often tempted by new
functionality into installing overprivileged
applications~\cite{android-demystified} or installing malware repackaged into
popular paid applications and sold for free on third-party markets. 

%Such ``sideloading'' of
%applications is a major reason for malware on smartphones today.

Even if users download apps only from trusted markets (such as Google Play)
and install only developer-signed binaries, apps can be compromised in the
field. Android Webviews enables developers to embed a webpage inside an
Android app. 
Researchers have shown
that Webviews is a rich source of vulnerabilities for malware to
exploit~\cite{webview-attacks}. Another major source of exploits in the wild are
third-party libraries that developers embed into their own applications. For
example, an advertisement library was recently discovered to be rife with
deliberate vulnerabilities~\cite{ad-vulna} that could be used by malware
to add malicious payloads to deployed applications.
}

%\parbold{Deployment.} 

%\name raises an alert if the signatures don't match.

%one to replay and analyze the traces, and one to use signatures for detecting
%malware from live traces. 

%More generally, 
%the trace collection component can either directly
%collect performance counters for each process instead of input trace.
\ignore{, or it can collect the minimal
user input and system information required to replay the execution for deeper analysis.
The replay component adds noise to the collected user inputs in order to generate a broader
training set. 
The analysis component then gets detailed performance counter traces (after replay)
and is trained to construct computational signatures for each application based on 
several variations of benign executions.
Finally, the detection component can use these signatures to compare with
signatures based on real live traces.
}
\ignore{
In this paper, we do not choose whether a component executes on client devices
or in a datacenter. Our primary goal is to determine whether computational
signatures are a viable option to tell benign-ware apart from malware. One
potential deployment scenario is that the signatures be generated in
datacenters that comprise of mobile devices (as used for testing mobile apps
today~\cite{testing-app}) and also analyzed in datacenters using light-weight
system call information recorded from client devices. Computational signatures
can be indexed by a unique app ID so that repackaged, renamed, or exploited
applications can be compared with signatures of the apps they purport to be.
}
%We assume that through social engineering or software exploits
%In particular, the baseline system can employ
%the default discretionary access control or mandatory access control policies (e.g.,
%SEAndroid) but malw


